QPS-r: A Cost-Effective Crossbar Scheduling Algorithm and Its Stability and Delay Analysis

In an input-queued switch, a crossbar schedule, or a matching between the input ports and the output ports needs to be computed in each switching cycle, or time slot. Designing switching algorithms with very low computational complexity, that lead to high throughput and small delay is a challenging problem. There appears to be a fundamental tradeoff between the computational complexity of the switching algorithm and the resultants throughput and delay. Parallel maximal matching algorithms (adapted for switching) appear to have stricken a sweet spot in this tradeoff, and prior work has shown the following performance guarantees. Using maximal matchings in every time slot results in at least 50% switch throughput and order-optimal (i.e., independent of the switch size N) average delay bounds for various traffic arrival processes. On the other hand, their computational complexity can be as low as $O(log^2N)$ per port/processor, which is much lower than those of the algorithms such as maximum weighted matching which ensures better throughput performance. In this work, we propose QPS-r, a parallel iterative switching algorithm that has the lowest possible computational complexity: O(1) per port. Using Lyapunov stability analysis, we show that the throughput and delay performance is identical to that of maximal matching algorithm. Although QPS-r builds upon an existing technique called Queue-Proportional Sampling (QPS), in this paper, we provide analytical guarantees on its throughput and delay under i.i.d. traffic as well as a Markovian traffic model which can model many realistic traffic patterns. We also demonstrate that QPS-3 (running 3 iterations) has comparable empirical throughput and delay performances as iSLIP (running $log_2 N$ iterations), a refined and optimized representative maximal matching algorithm adapted for switching.

==> sections/delay_analysis.tex <==
\subsection{Delay Analysis}\label{subsec: delay-analysis}

In this section, we derive the delay bounds for QPS-r. To prove the delay bound of QPS-r, we need the 
moment bound theorem~\cite[Proposition 2.1.4]{brucelecture2006}, stated as follows.

\begin{theorem}[Moment bound~\cite{brucelecture2006}]\label{thm:moment-bound}
Suppose that $\{Y_n\}_{n=0}^{\infty}$ is a positive recurrent Markov chain with countable state space $\mathcal{Y}$. Suppose $V$, $f$, and $g$ are non-negative functions on $\mathcal{Y}$ such that,
\begin{equation}
V(Y_{t+1}) -V(Y_{t})\leq -f(Y_{t}) + g(Y_{t}), \,\mbox{for all } Y_{t} \in \mathcal{Y}
\end{equation}
Then $\mathbb{E}[f(\hat{Y})]\leq \mathbb{E}[g(\hat{Y})]$, where $\hat{Y}$ is the stationary distribution of the Markov chain $\{Y\}_{n=0}^{\infty}$.
\end{theorem}

\begin{corollary}
For queueing system scheduling according to QPS-r, if the maximum load factor $\rho<1/2$, then 
the total average queue length satisfies,
\begin{equation}\label{eq:queue-length-bound}
\sum_{ij}\bar{q}_{ij} \leq \frac{\sum_{ij}\big{(}\sigma^2_{ij}-\lambda_{ij}\Lambda^\dagger_{ij} +\lambda_{ij}\big{)}}{2(1-2\rho)}.
\end{equation}
where $\sigma^2_{ij}=\mathbb{E}[a^2_{ij}(t)]-\lambda^2_{ij}$ is the variance of $a_{ij}(t)$, and 
$\bar{q}_{ij}\triangleq\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}q_{ij}(t)$.
\end{corollary}
\begin{IEEEproof}
Note that, the proof is almost the same as the proof of Theorem 2 in~\cite{Neely2008DelayMM}.
We reproduce it with some minor revisions for this paper to be self-contained.

Let $Y_t=\{Q(t), D(t)\}$, then Then $Y_t$ is a positive recurrent Markov chain (proved in~\autoref{subsec:throughput-analysis}). Define $V, f, g: \mathcal{Y}\rightarrow \mathbb{N}^{+}$ such that,
\begin{align*}
V(Y) &= L(Y)\\ f(Y)&=2\sum_{ij}q_{ij}\big{(}D^\dagger_{ij}(t)-A^\dagger_{ij}(t)\big{)}\\
g(Y)&=\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}.
\end{align*}

Then from~\autoref{eq:uncond-drift}, and based on~\autoref{thm:moment-bound}, we have,
\begin{align}
f(\hat{Y})\leq g(\hat{Y}).
\end{align}

From~\autoref{eq:bt}, $\bar{d}_{ij}\triangleq\lim_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}[d_{ij}(t)]=\lambda_{ij}$ (as $\{Q(t),S(t)\}_{t=0}^{\infty}$ is positive recurrent), we have,
\begin{equation}
2(1-2\rho)\sum_{ij}\hat{q}_{ij}\leq f(\hat{Y}) \leq g(\hat{Y}) \leq \sum_{ij}\big{(}\sigma^2_{ij}-\lambda_{ij}\Lambda^\dagger_{ij} + \lambda_{ij}\big{)}.
\end{equation}

Note that $\sum_{ij}\bar{q}_{ij}=\sum_{ij}\hat{q}_{ij}$, therefore,
\begin{equation}
\sum_{ij}\bar{q}_{ij}\leq \frac{\sum_{ij}\big{(}\sigma^2_{ij}-\lambda_{ij}\Lambda^\dagger_{ij} + \lambda_{ij}\big{)}}{2(1-2\rho)}.
\end{equation}



\end{IEEEproof}

\noindent
\medskip
{\bf Discussion.} Note that For Bernoulli {\it i.i.d.} traffic, we have $\sigma^2_{ij}=\lambda_{ij}-\lambda^2_{ij}$, hence,
\begin{align}
\sum_{ij}\bar{q}_{ij}&\leq \frac{\sum_{ij}\big{(}\sigma^2_{ij}-\lambda_{ij}\Lambda^\dagger_{ij} + \lambda_{ij}\big{)}}{2(1-2\rho)}\nonumber\\
&=\frac{\sum_{ij}\big{(}\sigma^2_{ij}-\lambda_{ij}(\Lambda_{i*}+\Lambda_{*j} -\lambda_{ij})+ \lambda_{ij}\big{)}}{2(1-2\rho)}.\nonumber\\
&\leq\frac{\sum_{ij}\big{(}\sigma^2_{ij} + \lambda^2_{ij} + \lambda_{ij}\big{)} }{2 (1 - 2\rho)}\nonumber\\
&=\frac{\sum_{ij}\lambda_{ij}}{1-2\rho}\nonumber\\
&\leq\frac{N\rho}{1 - 2\rho}.
\end{align}

By Little's Law, we can derive the average waiting delay under Bernoulli {\it i.i.d.} traffic satisfies 
\begin{equation}\label{eq:delay-bound}\bar{\omega}\leq \frac{1}{1-2\rho}.\end{equation}
Clearly it is independent of switch size, $N$.


==> sections/delay_analysis_OLD_.tex <==
\subsection{Delay Analysis}\label{subsec: delay-analysis}


In this section, we derive the delay bounds for QPS-1, which, we will show later, can 
directly apply to QPS-r. We first introduce 
the delay bound analysis for the maximal matching algorithms in~\cite{Neely2008DelayMM,Neely2009MMDelay}, 
based on which we then show that all the delay bounds derived in~\cite{Neely2008DelayMM,Neely2009MMDelay} 
also holds for QPS-1.

We first introduce some extra notations for the delay analysis in this work. 
For each VOQ$_{ij}$, we define its neighborhood as all the VOQs at its input and 
at its output, including itself. 
The total queue length of VOQs in the neighborhood is denoted $Q^\dagger_{ij}$. 
% Similarly for D\dagger_ij etc.  
% Let $Q^{\dagger}_{ij}(t)\triangleq Q_{i*}(t)+Q_{*j}(t)-q_{ij}(t)$ be the sum of the VOQ 
% lengths for the cross of the $i^{th}$ row and $j^{th}$ column of $Q(t)$, 
% here ``X'' stands for cross. 
% That is, $\hat{Q}_{ij}(t)$ is 
% the total VOQ length of all the VOQs, including  VOQ $j$ at input port $i$, that has contention with it. 
Similarly, we have $A^{\dagger}_{ij}(t), D^{\dagger}_{ij}(t)$, and $\Lambda^{\dagger}_{ij}$. 

\subsubsection{Delay Bound Analysis for Maximal Matchings}\label{subsubsec:mm-delay-bounds}

In~\cite{Neely2008DelayMM,Neely2009MMDelay}, M. Neely derived a series of delay bounds under different 
traffic patterns, by applying drift analysis method described 
in~\autoref{subsubsec:proof-technique} 
and using the following property of the maximal matching algorithms. 

\begin{equation}\label{eq:mm-property}
q_{ij}(t)D^{\dagger}_{ij}(t) - q_{ij}(t) \geq 0, \qquad \forall i,j.
\end{equation}

The above equation is because $D^{\dagger}_{ij}(t)$, the total departure for the cross of 
the $i^{th}$ row and $j^{th}$ column of the matrix $D(t)$, is at least $1$ for maximal 
matchings when $q_{ij}>0$, since otherwise we can add into the matching 
the edge between input port $i$ and output port $j$. 

More particularly, M. Neely first constructs the following Lyapunov function.
\begin{equation}\label{eq:neely-lyapunov}
L\big{(}Q(t)\big{)}=\frac{1}{2}\sum_{i,j}q_{ij}(t)Q^{\dagger}_{ij}(t).
\end{equation}

By analyzing the drift of \autoref{eq:neely-lyapunov}, M. Neely derives the following 
delay bound theorem for {\it i.i.d.} traffic. Note that M. Neely also derives 
delay bounds for other kinds of traffic patterns.

\begin{theorem}[Delay Bound Theorem~\cite{Neely2008DelayMM,Neely2009MMDelay}]\label{thm:delay-bound-neely}
Let $Q(t)$ be a queue length matrix of a switching system and L\big{(}Q(t)\big{)} is a Lyapunov 
function defined in~\autoref{eq:neely-lyapunov}. If the unconditional drift $\Delta(t)\triangleq\mathbb{E}\Big{[}L\big{(}Q(t+1)\big{)}-L\big{(}Q(t)\big{)}\Big{]}=\mathbb{E}\big{[}B(t)\big{]} - \sum_{i,j}\mathbb{E}\Big{[}q_{ij}(t)\big{(}D^{\dagger}_{ij}(t) - A^{\dagger}_{ij}(t)\big{)}\Big{]}$ satisfies the 
following property for any time slot $t$:
\begin{equation}\label{eq:drift-requirement-delay-bound}
\Delta(t)\leq \mathbb{E}\big{[}B(t)\big{)} - \sum_{i,j}\mathbb{E}\Big{[}q_{ij}(t) \big{(}1 - A^{\dagger}_{ij}(t)\big{)}\Big{]},
\end{equation}
where 
$B(t)=\frac{1}{2}\sum_{i,j}\big{(}a_{ij}(t)A^{\dagger}_{ij}(t)-2A^{\dagger}_{ij}(t)d_{ij}(t) + d_{ij}(t)\big{)}$.



Then, if the arrival process $A(t)$ is {\it i.i.d.} over different time slots and also independent of each VOQ, and it is in the 
stability region of the switching system, then the total average 
delay satisfies:
\begin{equation}\label{eq:delay-bound-nonburst}
\overline{W}\leq\frac{1 + \sum_{i,j}\big{(}\sigma_{ij}^2-\lambda_{ij}\Lambda^{\dagger}_{ij}\big{)}/\lambda_{tot}}{2(1 - \rho^*)},
\end{equation}
where $\lambda_{tot}\triangleq\sum_{ij}\lambda_{ij}$ is the total arrival rate, 
$\sigma_{ij}^2\triangleq\mathbb{E}\big{[}a_{ij}^2\big{]} - \lambda_{ij}^2$ is the variance
of $a_{ij}(t)$, and $\rho^*\triangleq\max_{i,j}\Lambda^{\dagger}_{ij}$.
\end{theorem}


\subsubsection{Delay Bound Analysis for QPS-1}\label{subsubsec:qps-1-delay-bounds}

% We first introduce some notations. [...] . Let $\hat{Q}_{ij}(t)=\sum_{(h,k)\in \mathcal{N}_{ij}}q_{hk}(t)$ in which 
% $\mathcal{N}_{ij}\triangleq\{(h,k) : h = i \text{ or } k = j\}$, using the terminology from graph theory, 
% is the set of all edges that are incident with (input port) $i$ or (output port) $j$. That is, $\hat{Q}_{ij}(t)$ is 
% the total VOQ length of all the VOQs, including  VOQ $j$ at input port $i$, that has contention with it. Similarly, 
% we can define $\hat{A}_{ij}(t), \hat{D}_{ij}(t)$, and $\hat{\lambda}_{ij}$. 


% \subsubsection{Theorem on Delay Bounds}

% We will rely on \autoref{thm:delay-bound-neely} to 
% prove the delay bounds of the QPS scheduling algorithm. 

% \begin{theorem}[Delay Bound Theorem~\cite{Neely2008DelayMM}]\label{thm:delay-bound-neely}
% Let $Q(t)$ be a queue length matrix of a switching system, and let 
% $L\big{(}Q(t)\big{)}=\frac{1}{2}\sum_{i,j}q_{ij}(t)\hat{Q}_{ij}(t)$ be a Lyapunov function 
% of $Q(t)$. If the unconditional drift $\Delta(t)\triangleq\mathbb{E}\Big{[}L\big{(}Q(t+1)\big{)}-L\big{(}Q(t)\big{)}\Big{]}$ satisfies the 
% following property for any time slot $t$:
% \begin{equation}\label{eq:drift-requirement-delay-bound}
% \Delta(t)\leq \mathbb{E}\big{[}B(t)\big{)} - \sum_{i,j}\mathbb{E}\Big{[}q_{ij}(t) \big{(}1 - \hat{A}_{ij}(t)\big{)}\Big{]},
% \end{equation}
% where 
% \[
% B(t)=\frac{1}{2}\sum_{i,j}\big{(}a_{ij}(t)\hat{A}_{ij}(t)-2\hat{A}_{ij}(t)d_{ij}(t) + d_{ij}(t)\big{)}.
% \]

% Then,
% \begin{enumerate}[(i)]
% \item If the arrival process $A(t)$ is {\it i.i.d.} over different time slots and also independent of each VOQ, and it is in the 
% stability region\footnote{to be added} of the switching system, then the total average 
% delay satisfies:
% % \[
% % \sum_{i,j}\bar{q}_{ij}\leq \frac{\mathbb{E}\big{[}a_{ij}(t)\hat{A}_{ij}(t)\big{]} - 2\lambda_{ij}\hat{\lambda}_{ij} + \lambda_{ij}}{2(1 - \rho^*)}
% % \]
% \begin{equation}\label{eq:delay-bound-nonburst}
% \overline{W}\leq\frac{1 + \sum_{i,j}\big{(}\sigma_{ij}^2-\lambda_{ij}\hat{\lambda}_{ij}\big{)}/\lambda_{tot}}{2(1 - \rho^*)},
% \end{equation}
% where $\lambda_{tot}\triangleq\sum_{ij}\lambda_{ij}$ is the total arrival rate, 
% $\sigma_{ij}^2\triangleq\mathbb{E}\big{[}a_{ij}^2\big{]} - \lambda_{ij}^2$ is the variance
% of $a_{ij}(t)$, and $\rho^*\triangleq\max_{i,j}\hat{\lambda}_{ij}$.
% \item If the arrival process is 2-state Markov modulated arrivals within the stability 
% region, and the Markov chains are independent of each other, then the total average delay 
% satisfies:
% \begin{align}
% \overline{W}\leq& \frac{1 + \frac{1}{2\lambda_{tot}}\sum_{i,j}\sigma_{ij}^2}{1 - \rho^*} \nonumber \\&+ \max_{i,j}\frac{1}{\beta_{ij} + \delta_{ij}}\Big{(}\frac{1 + \frac{1}{2\lambda_{tot}}\sum_{i,j}\theta_{ij}[1]}{1 - \rho^*}\Big{)}, \label{eq:delay-markov-modu}
% \end{align}
% where $\beta_{ij}, \delta_{ij}$ are the transition probability for the Markov chain of 
% VOQ $j$ at input port $i$, $\lambda_{tot}$ is the total arrival rate, and $\theta_{ij}[1]\triangleq\mathbb{E}\big{[}A_{ij}(t-1)A_{ij}(t)\big{]} - \lambda_{ij}^2$ is the 1-slot 
% auto-correlation for the process $A_{ij}(t)$.
% \end{enumerate}
% \end{theorem}


% -- Emphasis that, when the arrival is Poison the delay is $O(1)$ independent of $N$ 
% (compared to the $O(N)$ results of other analysis) and ON-OFF

% \subsubsection{Delay Bounds for QPS}


% In~\cite{Neely2008DelayMM}, Neely obtains the delay bounds for the maximal scheduling 
% by using the following property of it. For all $i, j=1,2,\cdots,N$, we have, for any time slot $t$, 
% \begin{equation}\label{eq:mm-property}
% q_{ij}(t)\hat{D}_{ij}(t)=q_{ij}(t)\sum_{(h,k)\in \mathcal{N}_{ij}}d_{hk}(t)\geq q_{ij}(t).
% \end{equation}

% Note that for the Lyapunov function $L\big{(}Q(t)\big{)}=\sum_{ij}q_{ij}(t)\hat{Q}_{ij}(t)$, 
% we have,
% \begin{equation}\label{eq:drift-neely}
% \Delta(t)=\mathbb{E}\big{[}B(t)\big{]} - \sum_{i,j}\mathbb{E}\Big{[}q_{ij}(t)\big{(}\hat{D}_{ij}(t) - \hat{A}_{ij}(t)\big{)}\Big{]}.
% \end{equation}

% Substituting \autoref{eq:mm-property} into \autoref{eq:drift-neely}, we can get the 
% the maximal scheduling satisfies \autoref{thm:delay-bound-neely} in 
% \autoref{thm:delay-bound-neely}. 

Unfortunately, QPS-1 does not satisfy property \autoref{eq:mm-property}. 
However, we find that QPS-1 satisfies a weaker condition than \autoref{eq:mm-property}.  
This weaker condition is specified in \autoref{lemma:QPS-property}, 
which can somehow be viewed as an expectation form of \autoref{eq:mm-property}. 
It is clear that \autoref{lemma:QPS-property} is enough for proving that 
QPS satisfies the requirement of \autoref{thm:delay-bound-neely}, 
{\it i.e.,} \autoref{eq:drift-requirement-delay-bound}.

\begin{lemma}\label{lemma:QPS-property}
Under the QPS scheduling algorithm, for any time slot $t$, we have,
\begin{equation}\label{eq:QPS-property}
\sum_{i,j}\mathbb{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t)- q_{ij}(t)\big{]}\geq 0.
\end{equation}
\end{lemma}

\begin{IEEEproof}
We first notice that,
\begin{equation}
\sum_{i,j}\mathbb{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t)\big{]}\!=\!\mathbb{E}\Big{[}\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\Big{]}.
\end{equation}
% Then, from the definition of $\hat{D}_{ij}(t)$, for any $i,j=1,2,\cdots,N$, we have, 
% \begin{equation}\label{eq:group-depart}
% \hat{D}_{ij}(t)=D_{i*}(t) + D_{*j}(t) - d_{ij}(t).
% \end{equation}

From the definition of $D^{\dagger}_{ij}(t)$, we have,
\begin{align}
&\sum_{,j}q_{ij}(t)D^{\dagger}_{ij}(t) \nonumber \\
=&\sum_{i,j}q_{ij}(t)\big{(}D_{i*}(t) + D_{*j}(t) - d_{ij}(t)\big{)} \nonumber \\
=&\sum_{i}Q_{i*}(t)D_{i*}(t) \!+\! \sum_{j}Q_{*j}(t)D_{*j}(t) \!-\!\sum_{i,j}q_{ij}(t)d_{ij}(t) \nonumber 
\end{align}

By simple calculations and using~\eqref{eq:departure-row} and \eqref{eq:departure-column}, 
we have, 

\begin{align}
&\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\nonumber \\
=&\sum_{i,j}q_{ij}(t)\widetilde{p}_{ij}(t) - \sum_{i,j}q_{ij}(t)\mathbb{E}\big{[}d_{ij}(t) \mid Q(t)\big{]}\nonumber\\
&+ \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{i,j}q_{ij}(t)\widetilde{p}_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)} + \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
\geq&\sum_{i,j}q_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}\prod_{k\neq i}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\nonumber\\
&+ \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{i,j}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}+\sum_{j=1}^{N}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{j}Q_{*j}(t)\Big{(}1 \!-\! \mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
&\!+\!\sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{j}Q_{*j}(t)=\sum_{i,j}q_{ij}(t)=\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)\mid Q(t)\big{]}. \nonumber
\end{align}

Therefore, we have property~\autoref{eq:QPS-property} holds.

% \begin{widetext}
% \begin{align}
% &\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)\hat{D}_{ij}(t) \mid Q(t)\big{]}\nonumber \\
% =&\sum_{i,j}q_{ij}(t)\widetilde{p}_{ij}(t) - \sum_{i,j}q_{ij}(t)\mathbb{E}\big{[}d_{ij}(t) \mid Q(t)\big{]} + \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \label{eq:qps-property-row-departure}\\
% =&\sum_{i,j}q_{ij}(t)\widetilde{p}_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)} + \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \label{eq:qps-property-conditional-p}\\
% \geq&\sum_{i,j}q_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}\prod_{k\neq i}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}+ \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \label{eq:qps-property-conditional-departure}\\
% =&\sum_{i,j}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}+ \sum_{j=1}^{N}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \label{eq:qps-property-column-departure}\\
% =&\sum_{j}Q_{*j}(t)\Big{(}1 - \mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]}\Big{)} +\sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
% =&\sum_{j}Q_{*j}(t)=\sum_{i,j}q_{ij}(t)=\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)\mid Q(t)\big{]}. \nonumber
% \end{align}
% \end{widetext}
%
% \autoref{eq:qps-property-row-departure} holds, because we have the linearity of expectation and \autoref{eq:departure-row}. 
% \autoref{eq:qps-property-conditional-p} holds because the definition of the conditional probability $\widetilde{p}_{ij}(t)$, 


% \autoref{eq:qps-property-conditional-departure} is because of \autoref{eq:accepting-prob}, and 
% \autoref{eq:qps-property-column-departure} is because of \autoref{eq:departure-column}.
\end{IEEEproof}

\subsubsection{Discussion}\label{subsec: discussion}
%
% {\bf I will emphasize that the delay bounds hold for QPS-r and it is constant for Poisson and Bernoulli i.i.d.}
%
Note that when the traffic is Bernoulli {\it i.i.d.} we have that $\sigma_{ij}\leq \lambda_{ij}$ 
for any $i,j$, therefore, the delay bound in~\autoref{eq:delay-bound-nonburst} can be relaxed as 
$\frac{1 - \sum_{i,j}\big{(}\lambda_{ij}\Lambda^{\dagger}_{ij}\big{)}/(2\lambda_{tot})}{1 - \rho^*}$. 
It is clear that this delay bound independent of the switch size, that is $O(1)$ with respective to 
the switch size.

Note also that like the throughput proof in~\autoref{subsec:throughput-analysis}, the delay 
proof also only uses the properties described in~\eqref{eq:departure-row} and \eqref{eq:departure-column}, which are clearly 
satisfied by QPS-r. Therefore, the delay bounds directly apply to QPS-r. 


==> sections/policy_and_analysis.tex <==
\section{QPS and Its Stability Analysis}\label{sec:qps-and-analysis}

In this section, we first review the QPS scheduling algorithm, which we first 
proposed in~\cite{Gong2017QPS} as an add-on approach for boosting the performance of 
existing input-queued crossbar scheduling algorithms, such as, iSLIP~\cite{McKeown99iSLIP} 
and SERENA~\cite{GiacconePrabhakarShah2003SERENA}. Then, we do the stability analysis for 
QPS working standalone. 

\subsection{QPS}\label{subsec:QPS}

QPS has two stages: a proposing stage and an accepting stage. For ease of presentation, we only 
present  the input port oriented version in which the input ports do the proposing while the 
output ports do the accepting. The output port oriented version is identical except that the 
output ports do the proposing and the input ports do the accepting.

In the proposing stage, each input port proposes to exactly one output port with a probability 
proportional to the queue length of the respective VOQ. Here we will only describe the operations 
at input port $1$, which are identical at any other input port. Denote as $m_1,m_2,\cdots,m_N$ 
the respective queue lengths of the $N$ VOQs at input port $1$, and as $m$ the total queue 
length ({\it i.e.,} $m=\sum_{k=1}^Nm_k$). Note that $m_k=0$ for $1 \leq k \leq N$ 
if VOQ $k$ is empty. Unless $m=0$, input port $1$ picks a VOQ proportionally, that is, 
it picks VOQ $k$ with the probability of $m_k/m$. It then proposes to output port $k$ ({\it i.e.,} 
the one corresponds to the VOQ it picks) with the value $m_k$ that will be used in the accepting 
stage. Note that if the accepting stage does not require the VOQ length information, then 
a single bit of ``1'' would be sent instead of the value of $m_k$.

In the accepting stage, depending on how many proposals an output port receives, it performs as follows.
\begin{enumerate}[{\bf Case }1.]
    \item {\bf No proposal.} Do nothing.
    \item {\bf One proposal.} Accept it ({\it e.g.,} sending a message, such as a bit of ``1'', 
    to notify it).
    \item {\bf More than one proposals.} Choose one and accept it. Note that as mentioned 
    in~\cite{Gong2017QPS}, there are many effective accepting policies, for example, the longest 
    VOQ first policy and proportional accepting policy described in~\cite{Gong2017QPS}. We will 
    show that, no matter which kind of accepting policies is used, 
    QPS can always guarantee strongly stable for the switched system as long as 
    the maximum load factor $\rho < 0.5$.
\end{enumerate}


\subsection{Stability Analysis}\label{subsec:stability-analysis}

Recall that $Q(t)=\big{(}q_{ij}(t)\big{)}$. Our technique is similar to the {\it queue grouping}~\cite{Wu2007QueueGrouping,Neely2008DelayMM,Dai00Speedup}. 
For each $1\leq i \leq N$, we define,
\begin{equation}\label{eq:rowsum}
Q_{i*}(t)=\sum_j q_{ij}(t).
\end{equation}

Clearly, $Q_{i*}(t)$ is the sum of queue lengths of all VOQs at input port $i$ during time slot $t$. 
Similarly, we define,
\begin{equation}\label{eq:columnsum}
Q_{*j}(t)=\sum_{i}q_{ij}(t).
\end{equation}

The stability analysis of QPS is accomplished by analyzing the Lyapunov function defined as follows.
\begin{equation}\label{eq:lyapunov}
L\big{(}Q(t)\big{)}=\sum_{i}Q_{i*}^2(t) + \sum_jQ_{*j}^2(t).
\end{equation}

For Lyapunov function~\autoref{eq:lyapunov}, we can establish the drift condition described in~\autoref{lemma:qps-drift}.

\begin{lemma}[Drift Under QPS]\label{lemma:qps-drift}
If QPS scheduling is applied in the input-queued switch every time slot, and the maximum load 
factor $\rho < 0.5$, then there exists $B,\epsilon >0$ such that, when $L\big{(}Q(t)\big{)} > B$, 
we have,
\begin{equation}\label{eq:qps-drift}
\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon\|Q(t)\|.
\end{equation}
\end{lemma}
\begin{IEEEproof}
First, we introduce some useful notations. 
Let $d_{ij}(t)$ be the number of packets depart from VOQ $j$ at input port $i$ during time slot $t$, 
$D_{i*}(t)=\sum_{j}d_{ij}(t)$, and $D_{*j}(t)=\sum_{i}d_{ij}(t)$. Similarly, let  
$\lambda_{i*}=\sum_{j}\lambda_{ij}$, $\lambda_{*j}=\sum_{i}\lambda_{ij}$, 
$A_{i*}(t)=\sum_{j}A_{ij}(t)$, and $A_{*j}(t)=\sum_{i}A_{ij}(t)$. 

Now, we can proceed with the proof. 
From \autoref{eq:queueing-dynamics-entrywise}, we have, for any $i$, 
\begin{equation}\label{eq:queue-dynamics-row}
Q_{i*}(t+1)=Q_{i*}(t) + A_{i*}(t) - D_{i*}(t),
\end{equation}
and for any $j$,
\begin{equation}\label{eq:queue-dynamics-column}
Q_{*j}(t+1)=Q_{*j}(t) + A_{*j}(t) - D_{*j}(t).
\end{equation}

By the description of the QPS policy in~\autoref{subsec:QPS}, we have, for any $i$,
\begin{equation}\label{eq:departure-row}
\mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \widetilde{p}_{ij}(t),
\end{equation}
where $\widetilde{p}_{ij}(t)$ is a conditional probability of the event that the proposal from 
input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the 
event that input port $i$ does propose to output port $j$, that is, input port $i$ picks 
VOQ $j$ in the proposing stage. Clearly, we have, for any $i,j$,
\begin{equation}\label{eq:cond-accept-p}
\widetilde{p}_{ij}(t)=\mathbb{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
\end{equation}

Similarly, we have, for any $j$,
\begin{equation}\label{eq:departure-column}
\mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
\end{equation}

After all the above preparations, we can proceed to analyze the drift of the Lyapunov function
~\autoref{eq:lyapunov}. Let us first deal with the drift of its first term, 
{\it i.e.,} $\sum_i Q^2_{i*}(t)$. 

% \begin{widetext}
% \begin{align}
% &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) - \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&\mathbb{E}\Big{[}\sum_i \big{(}A_{i*}(t) - D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) + A_{i*}(t) - D_{i*}(t)\big{)} 
% \mid Q(t) \Big{]} \label{eq:using-queue-dynamics}\\
% =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} + \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:using-arrival}\\
% =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \hat{p}_{ij}(t)\Big{)} + \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-depature}\\
% =&2\sum_{i}\lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \hat{p}_{ij}(t)\big{)}+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% \end{align}
% \end{widetext}
\begin{align}
&\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
=&\mathbb{E}\Big{[}\sum_i \big{(}A_{i*}(t) \!-\! D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) \!+\! A_{i*}(t) \!-\! D_{i*}(t)\big{)} 
\mid Q(t) \Big{]} \label{eq:using-queue-dynamics}\\
=&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\ 
&+ \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:using-arrival}\\
=&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \hat{p}_{ij}(t)\Big{)} \nonumber\\
&+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-depature}\\
=&2\sum_{i}\lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \hat{p}_{ij}(t)\big{)}\nonumber\\
&+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
\end{align}

\noindent
\textbf{Remarks}. {\it 1)} Equality in \autoref{eq:using-queue-dynamics} is due to the queueing dynamics in~\autoref{eq:queue-dynamics-row}. {\it 2)} Equality in \autoref{eq:using-arrival} uses the linearity of expectation and the fact that 
$\mathbb{E}\big{[}A_{i*}(t)\big{]}=\lambda_{i*}$ for any $i$ and $t$. {\it 3)} Equality in \autoref{eq:using-depature} is because of~\autoref{eq:departure-row}. {\it 4)} To avoid discussing the cases of ``dividing by zero'', we use the convention that $0/0=0$ in this 
proof. 

Similarly, we have,
% \begin{table*}[!htb]
% \centering
% \begin{minipage}{0.8\textwidth}

% \begin{widetext}
% \begin{align}
% % &\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&2\sum_{j}(\lambda_{*j} - 1) Q_{*j} + \sum_j \Big{(}Q_{*j}\prod_{i}\big{(}1 - \frac{Q_{ij}(t)}{Q_{i*}(t)}\big{)}\Big{)} \nonumber \\
% % &+ \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}
% &\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&2\sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) + \sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} 
% + \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:drift-term-2}
% \end{align}
% \end{widetext}
% \end{minipage}
% \end{table*}
\begin{align}
&\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
=&2\sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) + \sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} 
\nonumber\\
&+ \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:drift-term-2}
\end{align}

Because,
\[
|A_{i*}(t) - D_{i*}(t)| \leq A_{i*}(t) + 1.
\]
we have, there exists some constant $C_1$ such that for any $i$,
\begin{equation}\label{eq:bounded-moment-row}
\mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\leq \mathbb{E}\Big{[}\big{(}A_{i*}(t) \!+\! 1\big{)}^2 \Big{]}\!\leq\! \frac{C_1}{N}.
\end{equation}
Similarly, we have there exists some constant $C_2$ such that for any $j$,
\begin{equation}\label{eq:bounded-moment-column}
\mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\leq \frac{C_2}{N}.
\end{equation}

Now, we do some relaxation on $\widetilde{p}_{ij}(t)$, which is the probability that the proposal from 
input port $i$ is accepted by output port $j$ conditioning on that input port $i$ does propose 
to output port $j$. It is obvious that the proposal from input port $i$ {\bf has to} be accepted 
if it is the only proposal that output port $j$ receives. Therefore, we have, for any $i,j$,
\begin{equation}\label{eq:accepting-prob}
\widetilde{p}_{ij}(t)\geq \prod_{k\neq i} \big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)} \geq \prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}.
\end{equation}

Combining \autoref{eq:drift-term-1}, \autoref{eq:drift-term-2}, \autoref{eq:bounded-moment-row}, \autoref{eq:bounded-moment-column}, we have,

% \begin{widetext}
% \begin{align}
% &\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \nonumber \\
% \leq&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)
% -\sum_{i,j} \Big{(}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% +\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber\\
% =&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) 
% -\sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% +\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber \\
% =&2\Big{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\Big{)} + C_1 +C_2 \nonumber \\
% \leq&2(2\rho - 1)\|Q_{ij}(t)\|_1 + C_1 + C_2 \label{eq:arrival-adm}\\
% \leq&2(2\rho - 1)\|Q_{ij}(t)\| + C_1 + C_2. \label{eq:norm-rel}
% \end{align}
% \end{widetext}

\begin{align}
&\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \nonumber \\
\leq&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\nonumber\\
&-\sum_{i,j} \Big{(}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} \nonumber\\
&+\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber\\
=&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) \nonumber\\
&-\sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\nonumber\\
&+\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber \\
=&2\Big{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\Big{)} + C_1 +C_2 \nonumber \\
\leq&2(2\rho - 1)\|Q_{ij}(t)\|_1 + C_1 + C_2 \label{eq:arrival-adm}\\
\leq&2(2\rho - 1)\|Q_{ij}(t)\| + C_1 + C_2. \label{eq:norm-rel}
\end{align}

Clearly, if $\rho < \frac{1}{2}$, then there exists $\epsilon > 0$ and $B > 0$, when $L\big{(}Q(t)\big{)} > B$, we have,
\[
\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\leq -\epsilon\|Q(t)\|.
\]
\end{IEEEproof}


Combine \autoref{lemma:qps-drift} and {\bf Theorem 2} in~\cite{Leonardi2001Stability}, we can prove the stability 
of QPS, which is formally stated in~\autoref{thm:stability-qps}.

\begin{theorem}{Stability of QPS}\label{thm:stability-qps}
If the maximum load factor $\rho < 0.5$, then the switched system applying QPS every time 
slot is strongly stable.
\end{theorem}


==> sections/throughput_analysis-jxbak.tex <==
\section{Throughput and Delay Analysis}\label{sec:throughput-and-delay-analysis}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% This part of texts is an outline for this section
%% You can simply Line 16 of QPS.tex to noy include
%% this part.
\ifOutline
\fbox{\bf
\begin{minipage}[t]{0.45\textwidth}
\begin{center}{\color{red}$==========>$ outline $<===========$}\end{center}
\begin{enumerate}
\item Throughput analysis

A simple paragraph for the two commonly used proof techniques.

Prepare notations for Lyapunov function, then prove Lemma one followed by Theorem 1.

\item Delay analysis

A simple paragraph to describe Neely's proof. (summarize Neely's results in Theorem 2 \&
bring in the important property of maximal matching). Transit to QPS (from deterministic to
expectation). Prove the property of QPS and then discuss/explain their connections.

\end{enumerate}
\begin{center}
{\color{red}$======>$status: done $<========$}
\end{center}
\end{minipage}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% In this section, we prove that the QPS-r can achieve at least $50\%$
% throughput and derive its delay bounds. In~\autoref{subsec:background-notation},
% we introduce
% some background information and notations that we need in the stability proofs.
% In~\autoref{subsec:throughput-analysis}, we prove that QPS-r can achieve at least $50\%$
% throughput and derive its delay bounds in~\autoref{subsec: delay-analysis}.

% \subsection{Background and Notations}\label{subsec:background-notation}
\subsection{Preliminaries}\label{subsec:background-notation}\label{subsec:traffic-model}

% \subsubsection{Traffic Model}\label{subsec:traffic-model}

We first define three $N\times N$ matrices $Q(t)$, $A(t)$, and $D(t)$.
Let $Q(t) = \big{(}q_{ij}(t)\big{)}$ be the queue length matrix where $q_{ij}(t)$
is the length of the $j^{th}$ VOQ at input port $i$ during time slot $t$.
Let $A(t) = \big{(}a_{ij}(t)\big{)}$ be the traffic arrival matrix where $a_{ij}(t)$
is the number of packets arriving at the input port $i$ destined for
output port $j$ during time slot $t$.%, which can be viewed as the
counting process associated with underlying traffic arrival process.
Let $D(t) = \big{(}d_{ij}(t)\big{)}$ be the
departure matrix for time slot $t$ output by the crossbar scheduling algorithm.
Similar to $S(t)$, $D(t)$ is a $0$-$1$ matrix in which
$d_{ij}(t)=1$ if and only if there is a packet departing/transmitting
through VOQ$_{ij}$ during time slot $t$. Then, the queue length
matrix $Q$ evolves over time as follows.
\begin{equation}\label{eq:queueing-dynamics-entrywise}
q_{ij}(t + 1) = q_{ij}(t) - d_{ij}(t) + a_{ij}(t).
\end{equation}

Like in \cite{Gong2017QPS,Tassiulas90MaxWeight}, we assume that, for each $1\le i, j\le N$, $\{a_{ij}(t)\}_{t=0}^{\infty}$ is
a sequence of {\it i.i.d.} random variables,
%$i,j=1,2,\cdots,N$,
and the second moment
of their common distribution ($=\mathbb{E}\big{[}a^2_{ij}(0)\big{]}$) is finite.
% As mentioned above, our switch operates in slotted time, we assume that packets
% arrive at each input port can be modeled as a discrete-time Markov process. These discrete-time
% arrival processes can be characterized with an $N\times N$ matrix. Let $A(t)\!=\!\big{(}a_{ij}(t)\big{)}$
% denote this traffic arrival matrix in which $a_{ij}(t)$ is the amount of packets arriving to
% VOQ $j$ at the input port $i$ during time slot $t$.

Let $\lambda_{ij}$ be the normalized (to the percentage of the rate of an input/output link) mean arrival rate of packets to the $j^{th}$ VOQ (\ie those destined for
output port $j$) at input port $i$.  Then the
traffic pattern, can be represented by an $N \times N$ traffic matrix $\Lambda = \{\lambda_{ij}\}_{N\times N}$.
We also define $\rho$ as the maximum load factor imposed on any input or output port,
\begin{align}\label{def:lambda_max}
\rho \triangleq \max \big{\{} \max_{1\le i\le N}\{\lambda_i^{(in)}\}, \max_{1\le j\le N}\{\lambda_j^{(out)}\} \big{\}}
\end{align}
As mentioned before, we will prove %in~\autoref{sec:throughput-and-delay-analysis} 
in this section
that
QPS-r is stable and furthermore has good delay bound when the maximum load factor is less than half, i.e., 
$\rho < 1/2$.

\begin{comment}
We assume that, for any $1\leq i,j\leq N$,
$\big{\{}a_{ij}(\tau)\big{\}}_{\tau=1}^{\infty}$ is a sequence of independent and
identically distributed ({\it i.i.d.}) random variables of which the common distribution has
finite second moment, so that $\mathbb{E}\big{[}a^2_{ij}(t)\big{]}\!<\!\infty$ for any $t$.

Let $\lambda_{ij}=\mathbb{E}\big{[}a_{ij}(t)\big{]}$ be the average arrival rate to VOQ $j$ at input
port $i$. For ease of presentation in this paper, we define another $N\times N$ matrix, $\Lambda=\big{(}\lambda_{ij}\big{)}.
$We denote $\rho=\max\{\max_i \sum_j\lambda_{ij}, \max_j \sum_i \lambda_{ij}\}$ as the maximum load factor imposed on any input or output port. We will show later that
the switched system employing the QPS-r scheduling algorithm is stable (we will define it formally next)
whenever $\rho < 0.5$.

% \subsubsection{Queueing Dynamics}\label{subsec:queueing}

We define another two $N\times N$ matrices: $Q(t)$ and $S(t)$. Let $Q(t)\!=\!\big{(}q_{ij}(t)\big{)}$
be the queue length matrix in which $q_{ij}(t)$ denotes the number of packets
({\it i.e.,} VOQ length) buffered in VOQ $j$ at input port $i$ during time slot $t$. Similarly,
we denote $S(t)$ as the matching, or schedule during time slot $t$, that is, $s_{ij}(t)\!=\!1$ if
and only if input port $i$ matches with output port $j$ during time slot $i$, otherwise, $s_{ij}(t)=0$.
The queueing dynamics thus evolves as follows. For any $1\leq i,j\leq N$,
% \begin{equation}\label{eq:queueing-dynamics-entrywise-org}
% q_{ij}(t + 1) = \big{[}q_{ij}(t) + a_{ij}(t) - s_{ij}(t)\big{]}^{+}.
% \end{equation}
% remove (d(t)) dependency on a(t)
\begin{equation}\label{eq:queueing-dynamics-entrywise-org}
q_{ij}(t + 1) = \big{[}q_{ij}(t) - s_{ij}(t)\big{]}^{+} + a_{ij}(t) .
\end{equation}
where $[\cdot]^{+}\triangleq \max\{\cdot,0\}$.

For ease of analysis in this paper, we define another $N\times N$ $0$-$1$ matrix,
the departure matrix $D(t)=\big{(}d_{ij}(t)\big{)}$, in which $d_{ij}(t)$ is
the number of packets that is transmit from input port $i$ to output $j$. It is
clear that $d_{ij}=s_{ij}(t) \cdot 1_{\{q_{ij}(t) > 0\}}$ where
$1_{\{q_{ij}(t) > 0\}}$ is an indicator that equals $1$ if
$q_{ij}(t) > 0$ otherwise $0$. Therefore, the queueing dynamics equation
({\it i.e.,} \autoref{eq:queueing-dynamics-entrywise-org}) can be rewritten as,
\begin{equation}\label{eq:queueing-dynamics-entrywise}
q_{ij}(t + 1) = q_{ij}(t) - d_{ij}(t) + a_{ij}(t).
\end{equation}

\end{comment}
% \begin{definition}[Strongly Stable]\label{def:strongly-stable}
% A switched system with queue length matrix $\{Q(t)\}_{t=0}^{\infty}$ is {\bf strongly stable} if
% \[
% \lim\limits_{t\rightarrow \infty}\sup\mathbb{E}\big{[}\|Q(t)\|\big{]} < \infty,
% \]
% where $\|Q(t)\|=\sum_{i,j}q^2_{ij}(t)$.
% Note that this definition is the same as the one used
% in~\cite{Leonardi2001Stability}, which is slightly different from the one we used in our
% previous work~\cite{Gong2017QPS}. [equivalence]
% \end{definition}

\begin{comment}

\subsubsection{Proof Techniques}\label{subsubsec:proof-technique}

To show stability of a queueing system, there are two broad methods.
One is the fluid limit technique~\cite{Dai1995fluid}, and
the other is the Lyapunov function technique~\cite{Meyn2009BookMCSS}.
In this work, we are using the latter,
with which we construct a Lyapunov function, and
show that it has negative drift.
After that, we invoke {\bf Theorem 2} proved in~\cite{Leonardi2001Stability}, which
states that the queueing system is strongly stable if the negative drift
satisfies a stronger condition.

To further get the delay bounds of a queueing system, the general method is also
based on the Lyapunov function technique. One usually constructs a Lyapunov function,
which could be the same as or different than the one used in the stability proof.
And then analyze its unconditional drift, and by adding up infinite number of
such unconditional drift and using some Markov chain's properties,
the moment bound for the queue lengths is obtained.

[Prof. Siva maybe you can help me revise/add a few more high-level sentences on delay bound analysis
techniques]
\end{comment}


\subsection{Throughput Analysis}\label{subsec:throughput-analysis}

In this subsection we prove that QPS-r can achieve at least $50\%$ throughput.
The following theorem summarize the main results of this section.

% \subsubsection{Main Results}\label{subsubsec: main-res}
% \begin{theorem}[Stability of QPS-r]\label{thm:stability-qps}
% When the maximum load factor $\rho<1/2$,
% the switching system scheduling according to QPS-r every time
% slot is stable in the following stability notion.
% The joint queueing and scheduling process $\{Q(t), S(t)\}_{t=0}^{\infty}$
% is an ergodic Markov chain, and as a consequence,
% the queueing process $\{Q(t)\}_{t=0}^{\infty}$
% converges in distribution to a random matrix $\hat{Q}=\big{(}\hat{q}_{ij}\big{)}$. Furthermore,
% \[
% \mathbb{E}\big{[}\|\hat{Q}\|_1\big{]} < \infty.
% \]
% where $\|\hat{Q}\|_1=\sum_{i,j}\hat{q}_{ij}$.
% \end{theorem}

% Note that the stability notion in the above theorem
% is commonly used in previous work ({\it e.g.,} \cite{McKeownMekkittikulAnantharamEtAl1999,Mekkittikul98stability,Gong2017QPS,Tassiulas1998,GiacconePrabhakarShah2003SERENA}). To prove~\autoref{thm:stability-qps}, we need to show
% that (I) the Markov chain is positive recurrent and hence converges to a stationary distribution, and
% (II) the stationary distribution has a finite first moment.
\begin{theorem}[Stability of QPS-r]\label{thm:stability-qps}
When the maximum load factor $\rho<1/2$,
the switching system scheduling according to QPS-r every time
slot is stable in the following stability notion.
The joint queueing and scheduling process $\{Q(t), S(t)\}_{t=0}^{\infty}$
is a positive recurrent Markov chain.
\end{theorem}

By Foster-Lyapunov stability criterion~\cite[Proposition 2.1.1]{brucelecture2006}, to
prove the stability, we construct a Lyapunov function and obtain a negative drift
of it.
We accomplish the proof of the above theorem by analyzing the following Lyapunov function which was used in~\cite{Neely2008DelayMM, Neely2009MMDelay}, and is closely related to the Lyapunov function used in~\cite{Wu2007QueueGrouping,,Dai00Speedup,}.


% \begin{equation}\label{eq:lyapunov}
% L\big{(}Q(t)\big{)}=\sum_{i}Q_{i*}^2(t) + \sum_jQ_{*j}^2(t).
% \end{equation}
\begin{equation}\label{eq:lyapunov-org}
L\big{(}Q(t)\big{)}=\sum_{i,j}q_{ij}(t)\cdot\big{(}Q_{i*}(t) + Q_{*j}(t) - q_{ij}(t)\big{)}.
\end{equation}
where $Q_{i*}(t)$ and $Q_{*j}$ are the row sum of the $i^{th}$ row and
the column sum of the $j^{th}$
column of the queue length matrix $Q(t)$ respectively.
Mathematically, they are formally defined as follows.
\begin{align}
Q_{i*}(t)&=\sum_j q_{ij}(t) \label{eq:rowsum}\\
Q_{*j}(t)&=\sum_i q_{ij}(t). \label{eq:columnsum}
\end{align}
Note that this kind of notation applied to all other matrices defined in paper.
For example, $D_{i*}(t)$ denotes the row sum of the $i^{th}$ row of the departure
matrix $D(t)$.

For each VOQ$_{ij}$, we define its neighborhood as all the VOQs at its input and
at its output, including itself.
The total queue length at time slot $t$
of VOQs in the neighborhood is denoted $Q^\dagger_{ij}(t)$.
Clearly, $Q^\dagger_{ij}(t)=Q_{i*}(t) + Q_{*j}(t) - q_{ij}(t)$, hence the Lyapunov
function~\autoref{eq:lyapunov-org} can be re-written as,
\begin{equation}\label{eq:lyapunov}
L\big{(}Q(t)\big{)}=\sum_{i,j}q_{ij}(t)Q^\dagger_{ij}(t).
\end{equation}

The proof of~\autoref{thm:stability-qps} relies on the drift condition
of $L\big{(}Q(t)\big{)}$ stated in the following lemma.

\begin{lemma}[Drift Under QPS]\label{lemma:qps-drift}
If QPS scheduling is applied in the input-queued switch every time slot, and the maximum load
factor $\rho < 0.5$, then there exist $B,\epsilon >0$ such that, when $L\big{(}Q(t)\big{)} > B$,
we have,
\begin{equation}\label{eq:qps-drift}
\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon\|Q(t)\|_2.
\end{equation}
where $\|Q(t)\|_2=\sqrt{\sum_{ij}q^2_{ij}(t)}$ is the L2 norm of $Q(t)$.
\end{lemma}

To show the drift condition~\autoref{eq:qps-drift}, it relies on the following property of QPS-r.

\begin{lemma}[QPS-r Property]\label{lemma:QPS-property}
Under the QPS-r scheduling algorithm, for any time slot $t$, we have,
\begin{equation}\label{eq:QPS-property}
\sum_{i,j}\mathbb{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t)- q_{ij}(t)\big{]}\geq 0.
\end{equation}
\end{lemma}

We defer the proof of~\autoref{lemma:QPS-property} to~\autoref{subsubec:lemma-2-proof}.
Let us first recall the important property of
maximal matchings relating to it, which is commonly used in the previous work
({\it e.g.,} \cite{Neely2008DelayMM,Neely2009MMDelay,Dai00Speedup}) to analyze
the stability and delay bounds of queueing system scheduling according to maximal matchings.
That is $q_{ij}(t)D^{\dagger}_{ij}(t)- q_{ij}(t)\geq 0$, as $D^\dagger_{ij}(t)\geq 1$
when $q_{ij}(t)>0$ for maximal matchings. [A few sentences on the relation to be added.]

\subsection{Proof of~\autoref{lemma:qps-drift}}\label{subsubsec:proof-lemma-1}
% In this section, we prove~\autoref{lemma:qps-drift}.

% \begin{IEEEproof}
\begin{comment}
By simple calculations and using~\eqref{eq:queueing-dynamics-entrywise}, we have,
\begin{align}
&L\big{(}Q(t+1)\big{)} \nonumber \\
=&\sum_{ij}q_{ij}(t+1)Q^\dagger_{ij}(t+1)\nonumber\\
=&\sum_{ij}\big{(}q_{ij}(t)+a_{ij}(t)-d_{ij}(t)\big{)}\big{(}Q^\dagger_{ij}(t)+A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\nonumber\\
=&\sum_{ij}q_{ij}(t)Q^\dagger_{ij}(t) + \sum_{ij}q_{ij}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+ \sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}Q^\dagger_{ij}(t) \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:ltplusone}
\end{align}

Focus on the third term on the right-hand-side (RHS) of~\autoref{eq:ltplusone}, we have,
\begin{equation*}
\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}Q^\dagger_{ij}(t)\!=\!\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)-\sum_{ij}d_{ij}(t)Q^\dagger_{ij}(t)
\end{equation*}

Focus on the first term on the RHS of the above equation, we have,
\begin{align}
&\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)\nonumber\\
=&\sum_{ij}a_{ij}(t)\big{(}Q_{i*}(t)+Q_{*j}(t)-q_{ij}(t)\big{)}\nonumber\\
=&\sum_{ij}a_{ij}(t)Q_{i*}(t)\! +\! \sum_{ij}a_{ij}(t)Q_{*j}(t)\!-\!\sum_{ij}a_{ij}(t)q_{ij}(t)\label{eq:term-01}
\end{align}
Continue focusing the the first term on the RHS of the above equation, we have
\begin{align}
\sum_{ij}a_{ij}(t)Q_{i*}(t)&=\sum_{i}\big{(}Q_{i*}(t)\sum_{j}a_{ij}(t)\big{)}\nonumber\\
&=\sum_{i}Q_{i*}(t)A_{i*}(t)\nonumber\\
&=\sum_{i}\big{(}\sum_{j}q_{ij}(t)\big{)}A_{i*}(t)\nonumber\\
&=\sum_{ij}q_{ij}(t)A_{i*}(t)\label{eq:tterm-01}
\end{align}

Similarly, for the second term, we have,
\begin{equation}\label{eq:tterm-02}
\sum_{ij}a_{ij}(t)Q_{*j}(t)=\sum_{ij}q_{ij}(t)A_{*j}(t).
\end{equation}

Substitute \autoref{eq:tterm-01} and \autoref{eq:tterm-02} into \autoref{eq:term-01}, we have,
\begin{equation}\label{eq:term-a}
\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)=\sum_{ij}q_{ij}(t)A^\dagger_{ij}(t)
\end{equation}

Similarly, we have,
\begin{equation}\label{eq:term-d}
\sum_{ij}d_{ij}(t)Q^\dagger_{ij}(t)=\sum_{ij}q_{ij}(t)D^\dagger_{ij}(t)
\end{equation}

Substitute \autoref{eq:term-a} and \autoref{eq:term-d} into the third term on
the right-hand-side (RHS) of~\autoref{eq:ltplusone}, we have,
\begin{align}
&L\big{(}Q(t+1)\big{)}\nonumber\\
=&\sum_{ij}q_{ij}(t)Q^\dagger_{ij}(t) + 2\sum_{ij}q_{ij}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\nonumber\\
=&L\big{(}Q(t)\big{)}+ 2\sum_{ij}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:derived-drift}
\end{align}

Thus,
\end{comment}
%
It is not hard to check (for more detailed steps, please refer to~\cite{Neely2008DelayMM}),
\begin{align}
&L\big{(}Q(t+1)\big{)}-L\big{(}Q(t)\big{)}\nonumber\\
=&2\sum_{ij}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:uncond-drift}
\end{align}

Hence the drift of the Lyapunov function~\autoref{eq:lyapunov} can written as,
\begin{align}
&\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\nonumber\\
=&2\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} \nonumber\\
&+\sum_{ij}\mathbb{E}\Big{[}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} \label{eq:raw-drift}
\end{align}


To prove the negative drift of the Lyapunov function~\autoref{eq:lyapunov}, we will show that
the first term on the RHS of~\autoref{eq:raw-drift} is bounded by $2(2\rho-1)\|Q(t)\|_1$, and
the second one can be bounded by a constant for any fixed $N$. More formally, we will prove the
following two inequalities.
\begin{eqnarray}
\sum_{ij}\mathbb{E}\big{[}q_{ij}(t)\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\big{]}\!\leq\! (2\rho \!-\! 1)\|Q(t)\|_2.\label{eq:term-1-tbp}\\
\sum_{ij}\mathbb{E}\big{[}\big{(}a_{ij}(t)\!-\!d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\big{]} \!\leq\! CN^2,\label{eq:term-2-tbp}
\end{eqnarray}
where $C > 0$ is a constant.

First, let us focus on the proof of~\autoref{eq:term-1-tbp}, which is
a simple derivation based on~\autoref{lemma:QPS-property}, although
we will show later that the proof of~\autoref{lemma:QPS-property} is
quite involved, which we consider as one major contribution of this work.
Using the results of~\autoref{lemma:QPS-property}, we have,
\begin{align}
&\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\Big{]}\nonumber\\
=&\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)A^\dagger_{ij}(t) \Big{]}-\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)D^\dagger_{ij}(t)\Big{]}\nonumber\\
\leq&\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)A^\dagger_{ij}(t) \Big{]}-\sum_{ij}\mathbb{E}[q_{ij}(t)]\nonumber\\
=&\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)(A^\dagger_{ij}(t)-1)\Big{]}. \label{eq:bounded-first-term}
\end{align}

Now we proceed to prove~\autoref{eq:term-2-tbp}, similar proof can
be found in~\cite{Neely2008DelayMM}.
As $a_{ij}(t)$ is {\it i.i.d.} for any $i,j=1,2,\cdots,N$ (assumed in~\autoref{subsec:traffic-model}), we have,
\begin{align}
&\mathbb{E}\big{[}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\big{]}\nonumber\\
=&\mathbb{E}[a_{ij}(t)A^\dagger_{ij}(t) - d_{ij}(t)A^\dagger_{ij}(t)-a_{ij}(t)D^\dagger_{ij}(t)+d_{ij}(t)D^\dagger_{ij}(t)]\nonumber\\
=&\mathbb{E}[a^2_{ij}(t)]\!-\!\lambda^2_{ij}\!+\!\lambda_{ij}\Lambda^{\dagger}_{ij}
\!-\!\mathbb{E}[d_{ij}(t)]\Lambda^\dagger_{ij} \nonumber\\
&-\lambda_{ij}(t)\mathbb{E}[D^\dagger_{ij}(t)]\!+\! \mathbb{E}[d_{ij}(t)D^\dagger_{ij}(t)]\nonumber\\
=&\mathbb{E}[a^2_{ij}(t)]\!-\!\lambda^2_{ij}\!+\!\lambda_{ij}\Lambda^{\dagger}_{ij}
\!-\!\mathbb{E}[d_{ij}(t)]\Lambda^\dagger_{ij} \nonumber\\
&-\lambda_{ij}(t)\mathbb{E}[D^\dagger_{ij}(t)]\!+\! \mathbb{E}[d_{ij}(t)]. \label{eq:bt}
\end{align}

In the last step of the above derivation, we use the following fact of $D(t)$:
for any $i,j=1,2,\cdots,N$ we have $d_{ij}(t)D^\dagger_{ij}(t)= d_{ij}(t)$.
Because $d_{ij}(t)\in\{0,1\}$, and $D^\dagger_{ij}(t)= 1$ if $d_{ij}(t)=1$, otherwise $d_{ij}(t)D^\dagger_{ij}(t)=0=d_{ij}(t)$.

Recall (from~\autoref{subsec:traffic-model}) that $\mathbb{E}[a^2_{ij}(t)]<\infty$ (our assumption).
Besides $d_{ij}(t)\leq 1$, $D^\dagger_{ij}(t)\leq2$, $\lambda_{ij}\leq\rho<1/2$, and $\Lambda^\dagger_{ij}\leq 2\rho<1$, for all $i,j=1,2,\cdots,N$, hence there exist some constant $C>0$ such that,
\begin{equation*}
\mathbb{E}\Big{[}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} < C.
\end{equation*}

Therefore, for a fixed $N$, the second term of~\autoref{eq:raw-drift} is bounded,
\begin{equation}\label{eq:bounded-term}
\sum_{ij}\mathbb{E}\Big{[}\big{(}a_{ij}(t)\!-\!d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]}\!\leq\! CN^2.
\end{equation}


Now we can obtain the negative drift of~\autoref{lemma:qps-drift} by simply substituting~\autoref{eq:bounded-term} and \autoref{eq:bounded-first-term} into~\autoref{eq:raw-drift}.
\begin{align*}
&\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\nonumber\\
% \leq&2\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)(A^\dagger_{ij}(t)-1) \mid Q(t)\Big{]} + CN^2\nonumber\\
\leq&2(2\rho-1)\|Q(t)\|_1 + CN^2 \nonumber\\
=&-2(1 - 2\rho)\|Q(t)\|_1 + CN^2 \nonumber\\
\leq&-2(1 - 2\rho)\|Q(t)\|_2 + CN^2.
\end{align*}
In the last step we use the following well-known mathematical fact: for any finite dimension
vector $X$, we have $\|X\|_1\geq \|X\|_2$.

Therefore, we have, there exist $B,\epsilon >0$ such that, when $L\big{(}Q(t)\big{)} > B$,
\begin{equation*}
\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon\|Q(t)\|_2.
\end{equation*}

% \end{IEEEproof}
\noindent
{\bf Remarks.} The drift condition we obtained in the proof of~\autoref{lemma:qps-drift}
is stronger than the requirement of the Foster-Lyapunov stability
criterion~\cite[Proposition 2.1.1]{brucelecture2006}, which
only requires the drift
$\!\leq\! -\epsilon$ for some $\epsilon>0$ when $L\big{(}Q(t)\big{)} \!>\! B$.
With this stronger drift condition and using similar
approaches as in~\cite{Gong2017QPS,Tassiulas1998},
we can prove a stronger stability notion --
the first moment of the stationary distribution is bounded, {\it i.e.,}
$\|\hat{Q}\|_1\!<\!\infty$, where $\hat{Q}$ is the random matrix the
queueing process $\{Q(t)\}_{t=0}^{\infty}$ converges to in distribution.
Here, we skip the proof,
because we will prove next a even
stronger result -- the first moment of the stationary distribution
is bounded by some
constants for fixed $N$, furthermore the bound is $\frac{1}{1-2\rho}$
for Bernoulli {\it i.i.d.} traffic.

\subsection{Proof of \autoref{lemma:QPS-property}}\label{subsubec:lemma-2-proof}
In this section, we prove~\autoref{lemma:QPS-property}.
First, we analyze $\mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}$.
From the queue proportional sampling proposing strategy
described in~\autoref{subsubsec:qps-proposing}, we have, under
QPS-1, for any $i$,
\begin{equation}\label{eq:departure-row-org}
\mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
\end{equation}
where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
VOQ $j$ in the proposing stage. Clearly, we have, under QPS-1, for any $i,j$,
\begin{equation}\label{eq:cond-accept-p}
\alpha_{ij}(t)=\mathbb{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
\end{equation}

According to the description of QPS-r in~\autoref{subsec:qps-r}, we have, we have, under
QPS-r, for any $i$,
\begin{equation}\label{eq:departure-row}
\mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}\geq\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
\end{equation}

Similarly, we have, under QPS-r, for any $j$,
\begin{equation}\label{eq:departure-column}
\mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}\geq1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
\end{equation}
It is clear that the second term above is the probability that no input port
proposes to output port $j$. It is the only case that $D_{*j}(t)=0$, because
each input port proposes only when the corresponding VOQ is not empty and
according to the accepting strategy described
in~\autoref{subsubsec:qps-accepting}, as long as
there are proposal(s) output port $j$ would accept one (no matter which one).

Now we proceed to prove \autoref{lemma:QPS-property}.
\begin{IEEEproof}
We first notice that,
\begin{equation}
\sum_{i,j}\mathbb{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t)\big{]}\!=\!\mathbb{E}\Big{[}\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\Big{]}.
\end{equation}
% Then, from the definition of $\hat{D}_{ij}(t)$, for any $i,j=1,2,\cdots,N$, we have,
% \begin{equation}\label{eq:group-depart}
% \hat{D}_{ij}(t)=D_{i*}(t) + D_{*j}(t) - d_{ij}(t).
% \end{equation}

From the definition of $D^{\dagger}_{ij}(t)$, we have,
\begin{align}
&\sum_{,j}q_{ij}(t)D^{\dagger}_{ij}(t) \nonumber \\
=&\sum_{i,j}q_{ij}(t)\big{(}D_{i*}(t) + D_{*j}(t) - d_{ij}(t)\big{)} \nonumber \\
=&\sum_{i}Q_{i*}(t)D_{i*}(t) \!+\! \sum_{j}Q_{*j}(t)D_{*j}(t) \!-\!\sum_{i,j}q_{ij}(t)d_{ij}(t) \nonumber
\end{align}

By simple calculations and using~\eqref{eq:departure-row} and \eqref{eq:departure-column},
we have,

\begin{align}
&\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\nonumber \\
\geq&\sum_{i,j}q_{ij}(t)\alpha_{ij}(t) - \sum_{i,j}q_{ij}(t)\mathbb{E}\big{[}d_{ij}(t) \mid Q(t)\big{]}\nonumber\\
&+ \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{i,j}q_{ij}(t)\alpha_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)} + \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
\geq&\sum_{i,j}q_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}\prod_{k\neq i}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\nonumber\\
&+ \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{i,j}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}+\sum_{j=1}^{N}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
\geq&\sum_{j}Q_{*j}(t)\Big{(}1 \!-\! \mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
&\!+\!\sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{j}Q_{*j}(t)=\sum_{i,j}q_{ij}(t)=\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)\mid Q(t)\big{]}. \nonumber
\end{align}

Therefore, we have property~\autoref{eq:QPS-property} holds.
\end{IEEEproof}

% We first analyze the drift of the first term of the Lyapunov function~\eqref{eq:lyapunov}.
% By simple calculations and using~\eqref{eq:queueing-dynamics-entrywise}, we have,
% \begin{align}
% &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&\mathbb{E}\Big{[}\sum_i \big{(}A_{i*}(t) \!-\! D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) \!+\! A_{i*}(t) \!-\! D_{i*}(t)\big{)}
% \mid Q(t) \Big{]}\nonumber
% \end{align}

% Use the linearity of expectation and the fact that
% $\mathbb{E}\big{[}A_{i*}(t)\big{]}=\Lambda_{i*}$ for any $i$ and $t$, we have,
% \begin{align}
% &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\nonumber\\
% =&2\sum_{i}Q_{i*}(t)\Big{(}\Lambda_{i*} - \mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% &+ \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:first-term-using-avg-departure}
% \end{align}

% Let analyze the term $\mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}$ in the first term above.
% From the queue proportional sampling proposing strategy
% described in~\autoref{subsubsec:qps-proposing}, we have, for any $i$,
% \begin{equation}\label{eq:departure-row}
% \mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
% \end{equation}
% where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
% input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
% event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
% VOQ $j$ in the proposing stage. Clearly, we have, for any $i,j$,
% \begin{equation}\label{eq:cond-accept-p}
% \alpha_{ij}(t)=\mathbb{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
% \end{equation}

% % Similarly, we have, for any $j$,
% % \begin{equation}\label{eq:departure-column}
% % \mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% % \end{equation}

% Substitute~\autoref{eq:cond-accept-p} and \autoref{eq:departure-row}
% into \autoref{eq:first-term-using-avg-departure}, we have,
% \begin{align}
% &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&2\sum_{i}Q_{i*}(t)\Big{(}\Lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t)\Big{)} \nonumber\\
% &+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\nonumber\\
% =&2\sum_{i}\Lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \alpha_{ij}(t)\big{)}\nonumber\\
% &+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% \end{align}

% % From \autoref{eq:queueing-dynamics-entrywise}, we have, for any $i$,
% % \begin{equation}\label{eq:queue-dynamics-row}
% % Q_{i*}(t+1)=Q_{i*}(t) + A_{i*}(t) - D_{i*}(t),
% % \end{equation}
% % and for any $j$,
% % \begin{equation}\label{eq:queue-dynamics-column}
% % Q_{*j}(t+1)=Q_{*j}(t) + A_{*j}(t) - D_{*j}(t).
% % \end{equation}

% % By the description of the QPS policy in~\autoref{subsec:QPS},
% % From the queue proportional sampling proposing strategy
% % described in~\autoref{subsubsec:qps-proposing}, we have, for any $i$,
% % \begin{equation}\label{eq:departure-row}
% % \mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
% % \end{equation}
% % where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
% % input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
% % event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
% % VOQ $j$ in the proposing stage. Clearly, we have, for any $i,j$,
% % \begin{equation}\label{eq:cond-accept-p}
% % \alpha_{ij}(t)=\mathbb{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
% % \end{equation}

% % Similarly, we have, for any $j$,
% % \begin{equation}\label{eq:departure-column}
% % \mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% % \end{equation}

% % After all the above preparations, we can proceed to analyze the drift of the Lyapunov function
% % ~\autoref{eq:lyapunov}. Let us first deal with the drift of its first term,
% % {\it i.e.,} $\sum_i Q^2_{i*}(t)$.

% % \begin{widetext}
% % \begin{align}
% % &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) - \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&\mathbb{E}\Big{[}\sum_i \big{(}A_{i*}(t) - D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) + A_{i*}(t) - D_{i*}(t)\big{)}
% % \mid Q(t) \Big{]} \label{eq:using-queue-dynamics}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} + \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:using-arrival}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \hat{p}_{ij}(t)\Big{)} + \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-depature}\\
% % =&2\sum_{i}\lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \hat{p}_{ij}(t)\big{)}+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% % \end{align}
% % \end{widetext}
% % \begin{align}
% % &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&\mathbb{E}\Big{[}\sum_i \big{(}A_{i*}(t) \!-\! D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) \!+\! A_{i*}(t) \!-\! D_{i*}(t)\big{)}
% % \mid Q(t) \Big{]} \label{eq:using-queue-dynamics}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% % &+ \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:using-arrival}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \hat{p}_{ij}(t)\Big{)} \nonumber\\
% % &+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-depature}\\
% % =&2\sum_{i}\lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \hat{p}_{ij}(t)\big{)}\nonumber\\
% % &+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% % \end{align}

% % \noindent
% % \textbf{Remarks}. {\it 1)} Equality in \autoref{eq:using-queue-dynamics} is due to the queueing dynamics in~\autoref{eq:queue-dynamics-row}. {\it 2)} Equality in \autoref{eq:using-arrival} uses the linearity of expectation and the fact that
% % $\mathbb{E}\big{[}A_{i*}(t)\big{]}=\lambda_{i*}$ for any $i$ and $t$. {\it 3)} Equality in \autoref{eq:using-depature} is because of~\autoref{eq:departure-row}. {\it 4)} To avoid discussing the cases of ``dividing by zero'', we use the convention that $0/0=0$ in this
% % proof.

% Similarly, for the second term in the Lyapunov function~\eqref{eq:lyapunov}, we have,
% % \begin{table*}[!htb]
% % \centering
% % \begin{minipage}{0.8\textwidth}

% % \begin{widetext}
% % \begin{align}
% % % &\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% % % =&2\sum_{j}(\lambda_{*j} - 1) Q_{*j} + \sum_j \Big{(}Q_{*j}\prod_{i}\big{(}1 - \frac{Q_{ij}(t)}{Q_{i*}(t)}\big{)}\Big{)} \nonumber \\
% % % &+ \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}
% % &\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&2\sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) + \sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % + \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:drift-term-2}
% % \end{align}
% % \end{widetext}
% % \end{minipage}
% % \end{table*}
% \begin{align}
% &\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&2\sum_{j}Q_{*j}(t)\Big{(}\Lambda_{*j} - \mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% &+ \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-column-departure}\\
% =&2\sum_{j}(\Lambda_{*j} - 1) Q_{*j}(t) + \sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} \nonumber\\
% &+ \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:drift-term-2}
% \end{align}

% In the above derivation from \autoref{eq:using-column-departure} to \autoref{eq:drift-term-2},
% we use the following
% property of the column sum, $D_{*j}(t)$, of the departure matrix $D(t)$.
% \begin{equation}\label{eq:departure-column}
% \mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% \end{equation}
% It is clear that the second term above is the probability that no input port
% proposes to output port $j$. It is the only case that $D_{*j}(t)=0$, because
% each input port proposes only when the corresponding VOQ is not empty and
% according to the accepting strategy described
% in~\autoref{subsubsec:qps-accepting}, as long as
% there are proposal(s) output port $j$ would accept one (no matter which one).

% Now we proceed to analyze~\autoref{eq:drift-term-1}. Because,
% \[
% |A_{i*}(t) - D_{i*}(t)| \leq A_{i*}(t) + 1.
% \]
% and our assumption that each element of the arrival process $A(t)$ have
% a finite second moment in~\autoref{subsec:traffic-model},
% we have, there exists some constant $C_1$ such that for any $i$,
% \begin{equation}\label{eq:bounded-moment-row}
% \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\leq \mathbb{E}\Big{[}\big{(}A_{i*}(t) \!+\! 1\big{)}^2 \Big{]}\!\leq\! \frac{C_1}{N}.
% \end{equation}
% Similarly, we have there exists some constant $C_2$ such that for any $j$,
% \begin{equation}\label{eq:bounded-moment-column}
% \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\leq \frac{C_2}{N}.
% \end{equation}

% Now, we do some relaxation on $\alpha_{ij}(t)$, which is the probability that the proposal from
% input port $i$ is accepted by output port $j$ conditioning on that input port $i$ does propose
% to output port $j$. It is obvious that the proposal from input port $i$ {\bf has to} be accepted
% if it is the only proposal that output port $j$ receives. Therefore, we have, for any $i,j$,
% \begin{equation}\label{eq:accepting-prob}
% \alpha_{ij}(t)\geq \prod_{k\neq i} \big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)} \geq \prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}.
% \end{equation}

% Combining \autoref{eq:drift-term-1}, \autoref{eq:drift-term-2}, \autoref{eq:bounded-moment-row}, \autoref{eq:bounded-moment-column}, and \autoref{eq:accepting-prob}, we have,

% % \begin{widetext}
% % \begin{align}
% % &\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \nonumber \\
% % \leq&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)
% % -\sum_{i,j} \Big{(}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % +\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber\\
% % =&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)
% % -\sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % +\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber \\
% % =&2\Big{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\Big{)} + C_1 +C_2 \nonumber \\
% % \leq&2(2\rho - 1)\|Q_{ij}(t)\|_1 + C_1 + C_2 \label{eq:arrival-adm}\\
% % \leq&2(2\rho - 1)\|Q_{ij}(t)\| + C_1 + C_2. \label{eq:norm-rel}
% % \end{align}
% % \end{widetext}

% \begin{align}
% &\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \nonumber \\
% \leq&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\nonumber\\
% &-\sum_{i,j} \Big{(}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} \nonumber\\
% &+\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber\\
% =&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) \nonumber\\
% &-\sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\nonumber\\
% &+\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber \\
% =&2\Big{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\Big{)} + C_1 +C_2 \nonumber \\
% \leq&2(2\rho - 1)\|Q_{ij}(t)\|_1 + C_1 + C_2 \label{eq:arrival-adm}\\
% \leq&2(2\rho - 1)\|Q_{ij}(t)\| + C_1 + C_2. \label{eq:norm-rel}
% \end{align}

% Clearly, if $\rho < \frac{1}{2}$, then there exists $\epsilon > 0$ and $B > 0$, when $L\big{(}Q(t)\big{)} > B$, we have,
% \[
% \mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\leq -\epsilon\|Q(t)\|.
% \]
% \end{IEEEproof}

% As mentioned in~\autoref{subsubsec:proof-technique},
% combine \autoref{lemma:qps-drift} and {\bf Theorem 2}
% in~\cite{Leonardi2001Stability},
% we can prove the stability
% of QPS-1. That is, QPS-1 can achieve at least $50\%$ and furthermore the queueing
% system is strongly stable when the maximum load factor $\rho < 0.5$. Note that
% {\bf Theorem 2} in~\cite{Leonardi2001Stability} proves that any queueing system
% satisfying the drift condition~\autoref{eq:qps-drift} is strongly stable, the proof
% of which is somehow standard and has been done in other literature.

% It is clear that the above proof can be directly applied to QPS-r, with $r>1$, since
% ~\eqref{eq:departure-row} and \eqref{eq:departure-column} are clearly
% satisfied by QPS-r, which are the only properties of QPS-1 used in the proof.

% % which
% % can be viewed as as a special case of Tweedy's Theorem in~\cite[Theorem C.4]{Gong2017QPS}.
% % Similar theorems are commonly used in the crossbar scheduling literature~\cite{McKeownMekkittikulAnantharamEtAl1999,Mekkittikul98stability}.


% %\begin{comment}
% % move to other part
% % \begin{theorem}{Stability of QPS}\label{thm:stability-qps}
% % If the maximum load factor $\rho < 0.5$, then the switched system applying QPS every time
% % slot is strongly stable.
% % \end{theorem}
% %\end{comment} 

==> sections/throughput_analysis.tex <==
\section{Throughput and Delay Analysis}\label{sec:throughput-and-delay-analysis}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% This part of texts is an outline for this section
%% You can simply Line 16 of QPS.tex to noy include
%% this part.
\ifOutline
\fbox{\bf
\begin{minipage}[t]{0.45\textwidth}
\begin{center}{\color{red}$==========>$ outline $<===========$}\end{center}
\begin{enumerate}
\item Throughput analysis

A simple paragraph for the two commonly used proof techniques.

Prepare notations for Lyapunov function, then prove Lemma one followed by Theorem 1.

\item Delay analysis

A simple paragraph to describe Neely's proof. (summarize Neely's results in Theorem 2 \&
bring in the important property of maximal matching). Transit to QPS (from deterministic to
expectation). Prove the property of QPS and then discuss/explain their connections.

\end{enumerate}
\begin{center}
{\color{red}$======>$status: done $<========$}
\end{center}
\end{minipage}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% In this section, we prove that the QPS-r can achieve at least $50\%$
% throughput and derive its delay bounds. In~\autoref{subsec:background-notation},
% we introduce
% some background information and notations that we need in the stability proofs.
% In~\autoref{subsec:throughput-analysis}, we prove that QPS-r can achieve at least $50\%$
% throughput and derive its delay bounds in~\autoref{subsec: delay-analysis}.

% \subsection{Background and Notations}\label{subsec:background-notation}
\subsection{Preliminaries}\label{subsec:background-notation}\label{subsec:traffic-model}

% \subsubsection{Traffic Model}\label{subsec:traffic-model}

We first define three $N\times N$ matrices $Q(t)$, $A(t)$, and $D(t)$.
Let $Q(t) = \big{(}q_{ij}(t)\big{)}$ be the queue length matrix where $q_{ij}(t)$
is the length of the $j^{th}$ VOQ at input port $i$ during time slot $t$.
Let $A(t) = \big{(}a_{ij}(t)\big{)}$ be the traffic arrival matrix where $a_{ij}(t)$
is the number of packets arriving at the input port $i$ destined for
output port $j$ during time slot $t$.%, which can be viewed as the
counting process associated with underlying traffic arrival process.
Let $D(t) = \big{(}d_{ij}(t)\big{)}$ be the
departure matrix for time slot $t$ output by the crossbar scheduling algorithm.
Similar to $S(t)$, $D(t)$ is a $0$-$1$ matrix in which
$d_{ij}(t)=1$ if and only if there is a packet departing/transmitting
through VOQ$_{ij}$ during time slot $t$. Then, the queue length
matrix $Q$ evolves over time as follows.
\begin{equation}\label{eq:queueing-dynamics-entrywise}
q_{ij}(t + 1) = q_{ij}(t) - d_{ij}(t) + a_{ij}(t).
\end{equation}

Like in \cite{Gong2017QPS,Tassiulas90MaxWeight}, we assume that, for each $1\le i, j\le N$, $\{a_{ij}(t)\}_{t=0}^{\infty}$ is
a sequence of {\it i.i.d.} random variables,
%$i,j=1,2,\cdots,N$,
and the second moment
of their common distribution ($=\mathbf{E}\big{[}a^2_{ij}(0)\big{]}$) is finite.
% As mentioned above, our switch operates in slotted time, we assume that packets
% arrive at each input port can be modeled as a discrete-time Markov process. These discrete-time
% arrival processes can be characterized with an $N\times N$ matrix. Let $A(t)\!=\!\big{(}a_{ij}(t)\big{)}$
% denote this traffic arrival matrix in which $a_{ij}(t)$ is the amount of packets arriving to
% VOQ $j$ at the input port $i$ during time slot $t$.

Let $\lambda_{ij}$ be the normalized (to the percentage of the rate of an input/output link) mean arrival rate of packets to the $j^{th}$ VOQ (\ie those destined for
output port $j$) at input port $i$.  Then the
traffic pattern, can be represented by an $N \times N$ traffic matrix $\Lambda = \{\lambda_{ij}\}_{N\times N}$.
We also define $\rho$ as the maximum load factor imposed on any input or output port,
\begin{align}\label{def:lambda_max}
\rho \triangleq \max \big{\{} \max_{1\le i\le N}\{\lambda_i^{(in)}\}, \max_{1\le j\le N}\{\lambda_j^{(out)}\} \big{\}}
\end{align}
As mentioned before, we will prove %in~\autoref{sec:throughput-and-delay-analysis} 
in this section
that
QPS-r is stable and furthermore has good delay bound when the maximum load factor is less than half, i.e., 
$\rho < 1/2$.

\begin{comment}
We assume that, for any $1\leq i,j\leq N$,
$\big{\{}a_{ij}(\tau)\big{\}}_{\tau=1}^{\infty}$ is a sequence of independent and
identically distributed ({\it i.i.d.}) random variables of which the common distribution has
finite second moment, so that $\mathbf{E}\big{[}a^2_{ij}(t)\big{]}\!<\!\infty$ for any $t$.

Let $\lambda_{ij}=\mathbf{E}\big{[}a_{ij}(t)\big{]}$ be the average arrival rate to VOQ $j$ at input
port $i$. For ease of presentation in this paper, we define another $N\times N$ matrix, $\Lambda=\big{(}\lambda_{ij}\big{)}.
$We denote $\rho=\max\{\max_i \sum_j\lambda_{ij}, \max_j \sum_i \lambda_{ij}\}$ as the maximum load factor imposed on any input or output port. We will show later that
the switched system employing the QPS-r scheduling algorithm is stable (we will define it formally next)
whenever $\rho < 0.5$.

% \subsubsection{Queueing Dynamics}\label{subsec:queueing}

We define another two $N\times N$ matrices: $Q(t)$ and $S(t)$. Let $Q(t)\!=\!\big{(}q_{ij}(t)\big{)}$
be the queue length matrix in which $q_{ij}(t)$ denotes the number of packets
({\it i.e.,} VOQ length) buffered in VOQ $j$ at input port $i$ during time slot $t$. Similarly,
we denote $S(t)$ as the matching, or schedule during time slot $t$, that is, $s_{ij}(t)\!=\!1$ if
and only if input port $i$ matches with output port $j$ during time slot $i$, otherwise, $s_{ij}(t)=0$.
The queueing dynamics thus evolves as follows. For any $1\leq i,j\leq N$,
% \begin{equation}\label{eq:queueing-dynamics-entrywise-org}
% q_{ij}(t + 1) = \big{[}q_{ij}(t) + a_{ij}(t) - s_{ij}(t)\big{]}^{+}.
% \end{equation}
% remove (d(t)) dependency on a(t)
\begin{equation}\label{eq:queueing-dynamics-entrywise-org}
q_{ij}(t + 1) = \big{[}q_{ij}(t) - s_{ij}(t)\big{]}^{+} + a_{ij}(t) .
\end{equation}
where $[\cdot]^{+}\triangleq \max\{\cdot,0\}$.

For ease of analysis in this paper, we define another $N\times N$ $0$-$1$ matrix,
the departure matrix $D(t)=\big{(}d_{ij}(t)\big{)}$, in which $d_{ij}(t)$ is
the number of packets that is transmit from input port $i$ to output $j$. It is
clear that $d_{ij}=s_{ij}(t) \cdot 1_{\{q_{ij}(t) > 0\}}$ where
$1_{\{q_{ij}(t) > 0\}}$ is an indicator that equals $1$ if
$q_{ij}(t) > 0$ otherwise $0$. Therefore, the queueing dynamics equation
({\it i.e.,} \autoref{eq:queueing-dynamics-entrywise-org}) can be rewritten as,
\begin{equation}\label{eq:queueing-dynamics-entrywise}
q_{ij}(t + 1) = q_{ij}(t) - d_{ij}(t) + a_{ij}(t).
\end{equation}

\end{comment}
% \begin{definition}[Strongly Stable]\label{def:strongly-stable}
% A switched system with queue length matrix $\{Q(t)\}_{t=0}^{\infty}$ is {\bf strongly stable} if
% \[
% \lim\limits_{t\rightarrow \infty}\sup\mathbf{E}\big{[}\|Q(t)\|\big{]} < \infty,
% \]
% where $\|Q(t)\|=\sum_{i,j}q^2_{ij}(t)$.
% Note that this definition is the same as the one used
% in~\cite{Leonardi2001Stability}, which is slightly different from the one we used in our
% previous work~\cite{Gong2017QPS}. [equivalence]
% \end{definition}

\begin{comment}

\subsubsection{Proof Techniques}\label{subsubsec:proof-technique}

To show stability of a queueing system, there are two broad methods.
One is the fluid limit technique~\cite{Dai1995fluid}, and
the other is the Lyapunov function technique~\cite{Meyn2009BookMCSS}.
In this work, we are using the latter,
with which we construct a Lyapunov function, and
show that it has negative drift.
After that, we invoke {\bf Theorem 2} proved in~\cite{Leonardi2001Stability}, which
states that the queueing system is strongly stable if the negative drift
satisfies a stronger condition.

To further get the delay bounds of a queueing system, the general method is also
based on the Lyapunov function technique. One usually constructs a Lyapunov function,
which could be the same as or different than the one used in the stability proof.
And then analyze its unconditional drift, and by adding up infinite number of
such unconditional drift and using some Markov chain's properties,
the moment bound for the queue lengths is obtained.

[Prof. Siva maybe you can help me revise/add a few more high-level sentences on delay bound analysis
techniques]
\end{comment}

%%%%%%%% please move the proof of lemma 1 here
%%%%
%%%

\subsection{Throughput Analysis}\label{subsec:throughput-analysis}

In this subsection we prove that QPS-r can achieve at least $50\%$ throughput.
The following theorem summarize the main results of this section.

% \subsubsection{Main Results}\label{subsubsec: main-res}
% \begin{theorem}[Stability of QPS-r]\label{thm:stability-qps}
% When the maximum load factor $\rho<1/2$,
% the switching system scheduling according to QPS-r every time
% slot is stable in the following stability notion.
% The joint queueing and scheduling process $\{Q(t), S(t)\}_{t=0}^{\infty}$
% is an ergodic Markov chain, and as a consequence,
% the queueing process $\{Q(t)\}_{t=0}^{\infty}$
% converges in distribution to a random matrix $\hat{Q}=\big{(}\hat{q}_{ij}\big{)}$. Furthermore,
% \[
% \mathbf{E}\big{[}\|\hat{Q}\|_1\big{]} < \infty.
% \]
% where $\|\hat{Q}\|_1=\sum_{i,j}\hat{q}_{ij}$.
% \end{theorem}

% Note that the stability notion in the above theorem
% is commonly used in previous work ({\it e.g.,} \cite{McKeownMekkittikulAnantharamEtAl1999,Mekkittikul98stability,Gong2017QPS,Tassiulas1998,GiacconePrabhakarShah2003SERENA}). To prove~\autoref{thm:stability-qps}, we need to show
% that (I) the Markov chain is positive recurrent and hence converges to a stationary distribution, and
% (II) the stationary distribution has a finite first moment.
\begin{theorem}[Stability of QPS-r]\label{thm:stability-qps}
When the maximum load factor $\rho<1/2$,
the switching system scheduling according to QPS-r every time
slot is stable in the following notion:
The queueing process $\{Q(t)\}_{t=0}^{\infty}$
is a positive recurrent Markov chain.
\end{theorem}

By Foster-Lyapunov stability criterion~\cite[Proposition 2.1.1]{brucelecture2006}, to
prove the stability, we construct a Lyapunov function and obtain a negative drift
of it.
We accomplish the proof of the above theorem by analyzing the following Lyapunov function which was used in~\cite{Neely2008DelayMM, Neely2009MMDelay}, and is closely related to the Lyapunov function used in~\cite{Wu2007QueueGrouping,Dai00Speedup}.


% \begin{equation}\label{eq:lyapunov}
% L\big{(}Q(t)\big{)}=\sum_{i}Q_{i*}^2(t) + \sum_jQ_{*j}^2(t).
% \end{equation}
\begin{equation}\label{eq:lyapunov-org}
L\big{(}Q(t)\big{)}=\sum_{i,j}q_{ij}(t)\cdot\big{(}Q_{i*}(t) + Q_{*j}(t) - q_{ij}(t)\big{)}.
\end{equation}
where $Q_{i*}(t)$ and $Q_{*j}$ are the row sum of the $i^{th}$ row and
the column sum of the $j^{th}$
column of the queue length matrix $Q(t)$ respectively.
Mathematically, they are formally defined as follows.
\begin{align}
Q_{i*}(t)&=\sum_j q_{ij}(t) \label{eq:rowsum}\\
Q_{*j}(t)&=\sum_i q_{ij}(t). \label{eq:columnsum}
\end{align}
Note that this kind of notation applied to all other matrices defined in paper.
For example, $D_{i*}(t)$ denotes the row sum of the $i^{th}$ row of the departure
matrix $D(t)$.

For each VOQ$_{ij}$, we define its neighborhood as all the VOQs at its input and
at its output, including itself.
The total queue length at time slot $t$
of VOQs in the neighborhood is denoted $Q^\dagger_{ij}(t)$.
Clearly, $Q^\dagger_{ij}(t)=Q_{i*}(t) + Q_{*j}(t) - q_{ij}(t)$, hence the Lyapunov
function~\autoref{eq:lyapunov-org} can be re-written as,
\begin{equation}\label{eq:lyapunov}
L\big{(}Q(t)\big{)}=\sum_{i,j}q_{ij}(t)Q^\dagger_{ij}(t).
\end{equation}


Proof of Theorem 1 starts here -----------

Here we prove only the first part of the claim (that ... is positive recurrent), as the second part
(that ... < infinity) is implied by Theorem ?, which we will prove using some intermediate results
derived in this proof.   ...Q(t)... is clearly a Markov chain, since in (2), the term dijt is a function of 
Q(t) and aijt is a random variable independent of Q(t) 

To prove that ... is positive recurrent, it suffices to show that, there exists a constant $C > 0$ such that whenever $\|Q(t)\|_1 > C$, we have
\begin{equation}\label{eq:qps-drift}
\mathbf{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon
\end{equation}
where $\epsilon > 0$ is a constant.  


\begin{comment}
relies on the drift condition
of $L\big{(}Q(t)\big{)}$ stated in the following lemma.
\begin{lemma}[Drift Under QPS]\label{lemma:qps-drift}
If QPS scheduling is applied in the input-queued switch every time slot, and the maximum load
factor $\rho < 0.5$, then there exist $B,\epsilon >0$ such that, when $L\big{(}Q(t)\big{)} > B$,
we have,
\begin{equation}\label{eq:qps-drift}
\mathbf{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon\|Q(t)\|_2.
\end{equation}
where $\|Q(t)\|_2=\sqrt{\sum_{ij}q^2_{ij}(t)}$ is the L2 norm of $Q(t)$.
\end{lemma}
\end{comment}


\begin{comment}
%%%%%%%% moved to QPS-r property
To show the drift condition~\autoref{eq:qps-drift}, it relies on the following property of QPS-r.

\begin{lemma}[QPS-r Property]\label{lemma:QPS-property}
Under the QPS-r scheduling algorithm, for any time slot $t$, we have,
\begin{equation}\label{eq:QPS-property}
\sum_{i,j}\mathbf{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t)- q_{ij}(t)\big{]}\geq 0.
\end{equation}
\end{lemma}

We defer the proof of~\autoref{lemma:QPS-property} to~\autoref{subsubec:lemma-2-proof}.
Let us first recall the important property of
maximal matchings relating to it, which is commonly used in the previous work
({\it e.g.,} \cite{Neely2008DelayMM,Neely2009MMDelay,Dai00Speedup}) to analyze
the stability and delay bounds of queueing system scheduling according to maximal matchings.
That is $q_{ij}(t)D^{\dagger}_{ij}(t)- q_{ij}(t)\geq 0$, as $D^\dagger_{ij}(t)\geq 1$
when $q_{ij}(t)>0$ for maximal matchings. [A few sentences on the relation to be added.]

\end{comment}
\subsection{Proof of~\autoref{lemma:qps-drift}}\label{subsubsec:proof-lemma-1}
% In this section, we prove~\autoref{lemma:qps-drift}.

% \begin{IEEEproof}
\begin{comment}
By simple calculations and using~\eqref{eq:queueing-dynamics-entrywise}, we have,
\begin{align}
&L\big{(}Q(t+1)\big{)} \nonumber \\
=&\sum_{ij}q_{ij}(t+1)Q^\dagger_{ij}(t+1)\nonumber\\
=&\sum_{ij}\big{(}q_{ij}(t)+a_{ij}(t)-d_{ij}(t)\big{)}\big{(}Q^\dagger_{ij}(t)+A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\nonumber\\
=&\sum_{ij}q_{ij}(t)Q^\dagger_{ij}(t) + \sum_{ij}q_{ij}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+ \sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}Q^\dagger_{ij}(t) \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:ltplusone}
\end{align}

Focus on the third term on the right-hand-side (RHS) of~\autoref{eq:ltplusone}, we have,
\begin{equation*}
\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}Q^\dagger_{ij}(t)\!=\!\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)-\sum_{ij}d_{ij}(t)Q^\dagger_{ij}(t)
\end{equation*}

Focus on the first term on the RHS of the above equation, we have,
\begin{align}
&\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)\nonumber\\
=&\sum_{ij}a_{ij}(t)\big{(}Q_{i*}(t)+Q_{*j}(t)-q_{ij}(t)\big{)}\nonumber\\
=&\sum_{ij}a_{ij}(t)Q_{i*}(t)\! +\! \sum_{ij}a_{ij}(t)Q_{*j}(t)\!-\!\sum_{ij}a_{ij}(t)q_{ij}(t)\label{eq:term-01}
\end{align}
Continue focusing the the first term on the RHS of the above equation, we have
\begin{align}
\sum_{ij}a_{ij}(t)Q_{i*}(t)&=\sum_{i}\big{(}Q_{i*}(t)\sum_{j}a_{ij}(t)\big{)}\nonumber\\
&=\sum_{i}Q_{i*}(t)A_{i*}(t)\nonumber\\
&=\sum_{i}\big{(}\sum_{j}q_{ij}(t)\big{)}A_{i*}(t)\nonumber\\
&=\sum_{ij}q_{ij}(t)A_{i*}(t)\label{eq:tterm-01}
\end{align}

Similarly, for the second term, we have,
\begin{equation}\label{eq:tterm-02}
\sum_{ij}a_{ij}(t)Q_{*j}(t)=\sum_{ij}q_{ij}(t)A_{*j}(t).
\end{equation}

Substitute \autoref{eq:tterm-01} and \autoref{eq:tterm-02} into \autoref{eq:term-01}, we have,
\begin{equation}\label{eq:term-a}
\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)=\sum_{ij}q_{ij}(t)A^\dagger_{ij}(t)
\end{equation}

Similarly, we have,
\begin{equation}\label{eq:term-d}
\sum_{ij}d_{ij}(t)Q^\dagger_{ij}(t)=\sum_{ij}q_{ij}(t)D^\dagger_{ij}(t)
\end{equation}

Substitute \autoref{eq:term-a} and \autoref{eq:term-d} into the third term on
the right-hand-side (RHS) of~\autoref{eq:ltplusone}, we have,
\begin{align}
&L\big{(}Q(t+1)\big{)}\nonumber\\
=&\sum_{ij}q_{ij}(t)Q^\dagger_{ij}(t) + 2\sum_{ij}q_{ij}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\nonumber\\
=&L\big{(}Q(t)\big{)}+ 2\sum_{ij}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:derived-drift}
\end{align}

Thus,
\end{comment}




%
It is not hard to check (for more detailed steps, please refer to~\cite{Neely2008DelayMM}),
\begin{align}
&L\big{(}Q(t+1)\big{)}-L\big{(}Q(t)\big{)}\nonumber\\
=&2\sum_{ij}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:uncond-drift}
\end{align}

Hence the drift of the Lyapunov function~\autoref{eq:lyapunov} can written as,
\begin{align}
&\mathbf{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\nonumber\\
=&\mathbf{E}\Big{[}2\sum_{ij}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} \nonumber\\
&\mathbf{E}\Big{[}+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} \label{eq:raw-drift}
\end{align}

[to be moved further down]
Note that the LHS of ... and the LHS ... are the first term and the second term respectively in ... before the expectations are taken.  


To prove the negative drift of the Lyapunov function~\autoref{eq:lyapunov}, we will show that
the first term on the RHS of~\autoref{eq:raw-drift} is bounded by $2(2\rho-1)\|Q(t)\|_1$, and
the second one can be bounded by a constant for any fixed $N$. More formally, we will prove the
following two inequalities.


Now we claim following two inequalities, which we will prove shortly.
\begin{eqnarray}
\sum_{ij}\mathbf{E}\big{[}q_{ij}(t)\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\big{]}\!\leq\! (2\rho \!-\! 1)\|Q(t)\|_1\label{eq:term-1-tbp}\\
\sum_{ij}\mathbf{E}\big{[}\big{(}a_{ij}(t)\!-\!d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\big{]} \!\leq\! the detailed term \label{eq:term-2-tbp}
\end{eqnarray}

With ... and ..., we have 
$... < (2\rho \!-\! 1)\|Q(t)\|_1 + the detailed term$.  

%CN^2,
where $C > 0$ is a constant.

First, let us focus on the proof of~\autoref{eq:term-1-tbp}, which is
a simple derivation based on~\autoref{lemma:QPS-property}, although
we will show later that the proof of~\autoref{lemma:QPS-property} is
quite involved, which we consider as one major contribution of this work.
Using the results of~\autoref{lemma:QPS-property}, we have,
\begin{align}
&\sum_{ij}\mathbf{E}\Big{[}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\Big{]}\nonumber\\
=&\sum_{ij}\mathbf{E}\Big{[}q_{ij}(t)A^\dagger_{ij}(t) \Big{]}-\sum_{ij}\mathbf{E}\Big{[}q_{ij}(t)D^\dagger_{ij}(t)\Big{]}\nonumber\\
\leq&\sum_{ij}\mathbf{E}\Big{[}q_{ij}(t)A^\dagger_{ij}(t) \Big{]}-\sum_{ij}\mathbf{E}[q_{ij}(t)]\nonumber\\
=&\sum_{ij}\mathbf{E}\Big{[}q_{ij}(t)(A^\dagger_{ij}(t)-1)\Big{]}. \label{eq:bounded-first-term}
\end{align}

Now we proceed to prove~\autoref{eq:term-2-tbp}, similar proof can
be found in~\cite{Neely2008DelayMM}.
As $a_{ij}(t)$ is {\it i.i.d.} for any $i,j=1,2,\cdots,N$ (assumed in~\autoref{subsec:traffic-model}), we have,
\begin{align}
&\mathbf{E}\big{[}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\big{]}\nonumber\\
=&\mathbf{E}[a_{ij}(t)A^\dagger_{ij}(t) - d_{ij}(t)A^\dagger_{ij}(t)-a_{ij}(t)D^\dagger_{ij}(t)+d_{ij}(t)D^\dagger_{ij}(t)]\nonumber\\
=&\mathbf{E}[a^2_{ij}(t)]\!-\!\lambda^2_{ij}\!+\!\lambda_{ij}\Lambda^{\dagger}_{ij}
\!-\!\mathbf{E}[d_{ij}(t)]\Lambda^\dagger_{ij} \nonumber\\
&-\lambda_{ij}(t)\mathbf{E}[D^\dagger_{ij}(t)]\!+\! \mathbf{E}[d_{ij}(t)D^\dagger_{ij}(t)]\nonumber\\
=&\mathbf{E}[a^2_{ij}(t)]\!-\!\lambda^2_{ij}\!+\!\lambda_{ij}\Lambda^{\dagger}_{ij}
\!-\!\mathbf{E}[d_{ij}(t)]\Lambda^\dagger_{ij} \nonumber\\
&-\lambda_{ij}(t)\mathbf{E}[D^\dagger_{ij}(t)]\!+\! \mathbf{E}[d_{ij}(t)]. \label{eq:bt}
\end{align}

In the last step of the above derivation, we use the following fact of $D(t)$:
for any $i,j=1,2,\cdots,N$ we have $d_{ij}(t)D^\dagger_{ij}(t)= d_{ij}(t)$.
Because $d_{ij}(t)\in\{0,1\}$, and $D^\dagger_{ij}(t)= 1$ if $d_{ij}(t)=1$, otherwise $d_{ij}(t)D^\dagger_{ij}(t)=0=d_{ij}(t)$.

Recall (from~\autoref{subsec:traffic-model}) that $\mathbf{E}[a^2_{ij}(t)]<\infty$ (our assumption).
Besides $d_{ij}(t)\leq 1$, $D^\dagger_{ij}(t)\leq2$, $\lambda_{ij}\leq\rho<1/2$, and $\Lambda^\dagger_{ij}\leq 2\rho<1$, for all $i,j=1,2,\cdots,N$, hence there exist some constant $C>0$ such that,
\begin{equation*}
\mathbf{E}\Big{[}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} < C.
\end{equation*}

Therefore, for a fixed $N$, the second term of~\autoref{eq:raw-drift} is bounded,
\begin{equation}\label{eq:bounded-term}
\sum_{ij}\mathbf{E}\Big{[}\big{(}a_{ij}(t)\!-\!d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]}\!\leq\! CN^2.
\end{equation}


Now we can obtain the negative drift of~\autoref{lemma:qps-drift} by simply substituting~\autoref{eq:bounded-term} and \autoref{eq:bounded-first-term} into~\autoref{eq:raw-drift}.
\begin{align*}
&\mathbf{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\nonumber\\
% \leq&2\sum_{ij}\mathbf{E}\Big{[}q_{ij}(t)(A^\dagger_{ij}(t)-1) \mid Q(t)\Big{]} + CN^2\nonumber\\
\leq&2(2\rho-1)\|Q(t)\|_1 + CN^2 \nonumber\\
=&-2(1 - 2\rho)\|Q(t)\|_1 + CN^2 \nonumber\\
\leq&-2(1 - 2\rho)\|Q(t)\|_2 + CN^2.
\end{align*}
In the last step we use the following well-known mathematical fact: for any finite dimension
vector $X$, we have $\|X\|_1\geq \|X\|_2$.

Therefore, we have, there exist $B,\epsilon >0$ such that, when $L\big{(}Q(t)\big{)} > B$,
\begin{equation*}
\mathbf{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon\|Q(t)\|_2.
\end{equation*}

% \end{IEEEproof}
\noindent
{\bf Remarks.} The drift condition we obtained in the proof of~\autoref{lemma:qps-drift}
is stronger than the requirement of the Foster-Lyapunov stability
criterion~\cite[Proposition 2.1.1]{brucelecture2006}, which
only requires the drift
$\!\leq\! -\epsilon$ for some $\epsilon>0$ when $L\big{(}Q(t)\big{)} \!>\! B$.
With this stronger drift condition and using similar
approaches as in~\cite{Gong2017QPS,Tassiulas1998},
we can prove a stronger stability notion --
the first moment of the stationary distribution is bounded, {\it i.e.,}
$\|\hat{Q}\|_1\!<\!\infty$, where $\hat{Q}$ is the random matrix the
queueing process $\{Q(t)\}_{t=0}^{\infty}$ converges to in distribution.
Here, we skip the proof,
because we will prove next a even
stronger result -- the first moment of the stationary distribution
is bounded by some
constants for fixed $N$, furthermore the bound is $\frac{1}{1-2\rho}$
for Bernoulli {\it i.i.d.} traffic.

\subsection{Proof of \autoref{lemma:QPS-property}}\label{subsubec:lemma-2-proof}
In this section, we prove~\autoref{lemma:QPS-property}.
First, we analyze $\mathbf{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}$.
From the queue proportional sampling proposing strategy
described in~\autoref{subsubsec:qps-proposing}, we have, under
QPS-1, for any $i$,
\begin{equation}\label{eq:departure-row-org}
\mathbf{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
\end{equation}
where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
VOQ $j$ in the proposing stage. Clearly, we have, under QPS-1, for any $i,j$,
\begin{equation}\label{eq:cond-accept-p}
\alpha_{ij}(t)=\mathbf{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
\end{equation}

According to the description of QPS-r in~\autoref{subsec:qps-r}, we have, we have, under
QPS-r, for any $i$,
\begin{equation}\label{eq:departure-row}
\mathbf{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}\geq\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
\end{equation}

Similarly, we have, under QPS-r, for any $j$,
\begin{equation}\label{eq:departure-column}
\mathbf{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}\geq1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
\end{equation}
It is clear that the second term above is the probability that no input port
proposes to output port $j$. It is the only case that $D_{*j}(t)=0$, because
each input port proposes only when the corresponding VOQ is not empty and
according to the accepting strategy described
in~\autoref{subsubsec:qps-accepting}, as long as
there are proposal(s) output port $j$ would accept one (no matter which one).

Now we proceed to prove \autoref{lemma:QPS-property}.
\begin{IEEEproof}
It suffices to show that for any $i$ and $j$, we have 
\begin{equation}
\sum_{i,j}\mathbf{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]} \ge \sum_{i,j}q_{ij}(t) (label it)
\end{equation}
because with (label it), we have
\begin{equation}
\sum_{i,j}\mathbf{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t)\big{]}\!=\!\mathbf{E}\Big{[}\mathbf{E}\big{[}\sum_{i,j}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\Big{]}.
\end{equation}
$\ge \mathbf{E}\big{[}\sum_{i,j}q_{ij}(t)\big{]} = \sum_{i,j}\mathbf{E}\big{[}q_{ij}(t)\big{]} (Long, shift it to the right place)$
% Then, from the definition of $\hat{D}_{ij}(t)$, for any $i,j=1,2,\cdots,N$, we have,
% \begin{equation}\label{eq:group-depart}
% \hat{D}_{ij}(t)=D_{i*}(t) + D_{*j}(t) - d_{ij}(t).
% \end{equation}

From the definition of $D^{\dagger}_{ij}(t)$, we have,
\begin{align}
&\sum_{,j}q_{ij}(t)D^{\dagger}_{ij}(t) \nonumber \\
=&\sum_{i,j}q_{ij}(t)\big{(}D_{i*}(t) - d_{ij}(t) + D_{*j}(t)\big{)} \nonumber \\
=&\sum_{i}Q_{i*}(t)D_{i*}(t) \!-\!\sum_{i,j}q_{ij}(t)d_{ij}(t) \!+\! \sum_{j}Q_{*j}(t)D_{*j}(t) \nonumber
\end{align}

By simple calculations and using~\eqref{eq:departure-row} and \eqref{eq:departure-column},
we have,

\begin{align}
&\sum_{i,j} \mathbf{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\nonumber \\
=&\sum_{i,j} q_{ij}(t)\mathbf{E}\big{[}D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\nonumber \\
=&\sum_{i,j} q_{ij}(t)\mathbf{E}\big{[}D_{i*}(t) - d_{ij}(t) + D_{*j}(t)  \mid Q(t)\big{]}\nonumber \\
=& summaton-of-three-conditional-expectations \nonumber \\
=&\sum_{i}Q_{i*}(t)\mathbf{E}\big{[}D_{i*}(t)\mid Q(t)\big{]} \!-\!\sum_{i,j} q_{ij}(t) \mathbf{E}\big{[}d_{ij}(t)\mid Q(t)\big{]} \!+\! \sum_{j} Q_{*j}(t)\mathbf{E}\big{[}D_{*j}(t) \mid Q(t)\big{]} \nonumber\\
\geq&\sum_{i,j}q_{ij}(t)\alpha_{ij}(t) - \sum_{i,j}q_{ij}(t)\mathbf{E}\big{[}d_{ij}(t) \mid Q(t)\big{]}\nonumber\\
&+ \sum_{j}Q_{*j}(t)\mathbf{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{i,j}q_{ij}(t)\alpha_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)} + \sum_{j}Q_{*j}(t)\mathbf{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
\geq&\sum_{i,j}q_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}\prod_{k\neq i}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\nonumber\\
&+ \sum_{j}Q_{*j}(t)\mathbf{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{i,j}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}+\sum_{j=1}^{N}Q_{*j}(t)\mathbf{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
\geq&\sum_{j}Q_{*j}(t)\Big{(}1 \!-\! \mathbf{E}\big{[}D_{*j}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
&\!+\!\sum_{j}Q_{*j}(t)\mathbf{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{j}Q_{*j}(t)=\sum_{i,j}q_{ij}(t)=\mathbf{E}\big{[}\sum_{i,j}q_{ij}(t)\mid Q(t)\big{]}. \nonumber
\end{align}

Therefore, we have property~\autoref{eq:QPS-property} holds.
\end{IEEEproof}

% We first analyze the drift of the first term of the Lyapunov function~\eqref{eq:lyapunov}.
% By simple calculations and using~\eqref{eq:queueing-dynamics-entrywise}, we have,
% \begin{align}
% &\mathbf{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&\mathbf{E}\Big{[}\sum_i \big{(}A_{i*}(t) \!-\! D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) \!+\! A_{i*}(t) \!-\! D_{i*}(t)\big{)}
% \mid Q(t) \Big{]}\nonumber
% \end{align}

% Use the linearity of expectation and the fact that
% $\mathbf{E}\big{[}A_{i*}(t)\big{]}=\Lambda_{i*}$ for any $i$ and $t$, we have,
% \begin{align}
% &\mathbf{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\nonumber\\
% =&2\sum_{i}Q_{i*}(t)\Big{(}\Lambda_{i*} - \mathbf{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% &+ \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:first-term-using-avg-departure}
% \end{align}

% Let analyze the term $\mathbf{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}$ in the first term above.
% From the queue proportional sampling proposing strategy
% described in~\autoref{subsubsec:qps-proposing}, we have, for any $i$,
% \begin{equation}\label{eq:departure-row}
% \mathbf{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
% \end{equation}
% where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
% input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
% event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
% VOQ $j$ in the proposing stage. Clearly, we have, for any $i,j$,
% \begin{equation}\label{eq:cond-accept-p}
% \alpha_{ij}(t)=\mathbf{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
% \end{equation}

% % Similarly, we have, for any $j$,
% % \begin{equation}\label{eq:departure-column}
% % \mathbf{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% % \end{equation}

% Substitute~\autoref{eq:cond-accept-p} and \autoref{eq:departure-row}
% into \autoref{eq:first-term-using-avg-departure}, we have,
% \begin{align}
% &\mathbf{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&2\sum_{i}Q_{i*}(t)\Big{(}\Lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t)\Big{)} \nonumber\\
% &+ \sum_i \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\nonumber\\
% =&2\sum_{i}\Lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \alpha_{ij}(t)\big{)}\nonumber\\
% &+ \sum_i \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% \end{align}

% % From \autoref{eq:queueing-dynamics-entrywise}, we have, for any $i$,
% % \begin{equation}\label{eq:queue-dynamics-row}
% % Q_{i*}(t+1)=Q_{i*}(t) + A_{i*}(t) - D_{i*}(t),
% % \end{equation}
% % and for any $j$,
% % \begin{equation}\label{eq:queue-dynamics-column}
% % Q_{*j}(t+1)=Q_{*j}(t) + A_{*j}(t) - D_{*j}(t).
% % \end{equation}

% % By the description of the QPS policy in~\autoref{subsec:QPS},
% % From the queue proportional sampling proposing strategy
% % described in~\autoref{subsubsec:qps-proposing}, we have, for any $i$,
% % \begin{equation}\label{eq:departure-row}
% % \mathbf{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
% % \end{equation}
% % where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
% % input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
% % event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
% % VOQ $j$ in the proposing stage. Clearly, we have, for any $i,j$,
% % \begin{equation}\label{eq:cond-accept-p}
% % \alpha_{ij}(t)=\mathbf{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
% % \end{equation}

% % Similarly, we have, for any $j$,
% % \begin{equation}\label{eq:departure-column}
% % \mathbf{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% % \end{equation}

% % After all the above preparations, we can proceed to analyze the drift of the Lyapunov function
% % ~\autoref{eq:lyapunov}. Let us first deal with the drift of its first term,
% % {\it i.e.,} $\sum_i Q^2_{i*}(t)$.

% % \begin{widetext}
% % \begin{align}
% % &\mathbf{E}\big{[}\sum_{i}Q_{i*}^2(t+1) - \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&\mathbf{E}\Big{[}\sum_i \big{(}A_{i*}(t) - D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) + A_{i*}(t) - D_{i*}(t)\big{)}
% % \mid Q(t) \Big{]} \label{eq:using-queue-dynamics}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \mathbf{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} + \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:using-arrival}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \hat{p}_{ij}(t)\Big{)} + \sum_i \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-depature}\\
% % =&2\sum_{i}\lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \hat{p}_{ij}(t)\big{)}+ \sum_i \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% % \end{align}
% % \end{widetext}
% % \begin{align}
% % &\mathbf{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&\mathbf{E}\Big{[}\sum_i \big{(}A_{i*}(t) \!-\! D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) \!+\! A_{i*}(t) \!-\! D_{i*}(t)\big{)}
% % \mid Q(t) \Big{]} \label{eq:using-queue-dynamics}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \mathbf{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% % &+ \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:using-arrival}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \hat{p}_{ij}(t)\Big{)} \nonumber\\
% % &+ \sum_i \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-depature}\\
% % =&2\sum_{i}\lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \hat{p}_{ij}(t)\big{)}\nonumber\\
% % &+ \sum_i \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% % \end{align}

% % \noindent
% % \textbf{Remarks}. {\it 1)} Equality in \autoref{eq:using-queue-dynamics} is due to the queueing dynamics in~\autoref{eq:queue-dynamics-row}. {\it 2)} Equality in \autoref{eq:using-arrival} uses the linearity of expectation and the fact that
% % $\mathbf{E}\big{[}A_{i*}(t)\big{]}=\lambda_{i*}$ for any $i$ and $t$. {\it 3)} Equality in \autoref{eq:using-depature} is because of~\autoref{eq:departure-row}. {\it 4)} To avoid discussing the cases of ``dividing by zero'', we use the convention that $0/0=0$ in this
% % proof.

% Similarly, for the second term in the Lyapunov function~\eqref{eq:lyapunov}, we have,
% % \begin{table*}[!htb]
% % \centering
% % \begin{minipage}{0.8\textwidth}

% % \begin{widetext}
% % \begin{align}
% % % &\mathbf{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% % % =&2\sum_{j}(\lambda_{*j} - 1) Q_{*j} + \sum_j \Big{(}Q_{*j}\prod_{i}\big{(}1 - \frac{Q_{ij}(t)}{Q_{i*}(t)}\big{)}\Big{)} \nonumber \\
% % % &+ \sum_j \mathbf{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}
% % &\mathbf{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&2\sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) + \sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % + \sum_j \mathbf{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:drift-term-2}
% % \end{align}
% % \end{widetext}
% % \end{minipage}
% % \end{table*}
% \begin{align}
% &\mathbf{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&2\sum_{j}Q_{*j}(t)\Big{(}\Lambda_{*j} - \mathbf{E}\big{[}D_{*j}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% &+ \mathbf{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-column-departure}\\
% =&2\sum_{j}(\Lambda_{*j} - 1) Q_{*j}(t) + \sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} \nonumber\\
% &+ \sum_j \mathbf{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:drift-term-2}
% \end{align}

% In the above derivation from \autoref{eq:using-column-departure} to \autoref{eq:drift-term-2},
% we use the following
% property of the column sum, $D_{*j}(t)$, of the departure matrix $D(t)$.
% \begin{equation}\label{eq:departure-column}
% \mathbf{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% \end{equation}
% It is clear that the second term above is the probability that no input port
% proposes to output port $j$. It is the only case that $D_{*j}(t)=0$, because
% each input port proposes only when the corresponding VOQ is not empty and
% according to the accepting strategy described
% in~\autoref{subsubsec:qps-accepting}, as long as
% there are proposal(s) output port $j$ would accept one (no matter which one).

% Now we proceed to analyze~\autoref{eq:drift-term-1}. Because,
% \[
% |A_{i*}(t) - D_{i*}(t)| \leq A_{i*}(t) + 1.
% \]
% and our assumption that each element of the arrival process $A(t)$ have
% a finite second moment in~\autoref{subsec:traffic-model},
% we have, there exists some constant $C_1$ such that for any $i$,
% \begin{equation}\label{eq:bounded-moment-row}
% \mathbf{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\leq \mathbf{E}\Big{[}\big{(}A_{i*}(t) \!+\! 1\big{)}^2 \Big{]}\!\leq\! \frac{C_1}{N}.
% \end{equation}
% Similarly, we have there exists some constant $C_2$ such that for any $j$,
% \begin{equation}\label{eq:bounded-moment-column}
% \mathbf{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\leq \frac{C_2}{N}.
% \end{equation}

% Now, we do some relaxation on $\alpha_{ij}(t)$, which is the probability that the proposal from
% input port $i$ is accepted by output port $j$ conditioning on that input port $i$ does propose
% to output port $j$. It is obvious that the proposal from input port $i$ {\bf has to} be accepted
% if it is the only proposal that output port $j$ receives. Therefore, we have, for any $i,j$,
% \begin{equation}\label{eq:accepting-prob}
% \alpha_{ij}(t)\geq \prod_{k\neq i} \big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)} \geq \prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}.
% \end{equation}

% Combining \autoref{eq:drift-term-1}, \autoref{eq:drift-term-2}, \autoref{eq:bounded-moment-row}, \autoref{eq:bounded-moment-column}, and \autoref{eq:accepting-prob}, we have,

% % \begin{widetext}
% % \begin{align}
% % &\mathbf{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \nonumber \\
% % \leq&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)
% % -\sum_{i,j} \Big{(}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % +\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber\\
% % =&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)
% % -\sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % +\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber \\
% % =&2\Big{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\Big{)} + C_1 +C_2 \nonumber \\
% % \leq&2(2\rho - 1)\|Q_{ij}(t)\|_1 + C_1 + C_2 \label{eq:arrival-adm}\\
% % \leq&2(2\rho - 1)\|Q_{ij}(t)\| + C_1 + C_2. \label{eq:norm-rel}
% % \end{align}
% % \end{widetext}

% \begin{align}
% &\mathbf{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \nonumber \\
% \leq&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\nonumber\\
% &-\sum_{i,j} \Big{(}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} \nonumber\\
% &+\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber\\
% =&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) \nonumber\\
% &-\sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\nonumber\\
% &+\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber \\
% =&2\Big{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\Big{)} + C_1 +C_2 \nonumber \\
% \leq&2(2\rho - 1)\|Q_{ij}(t)\|_1 + C_1 + C_2 \label{eq:arrival-adm}\\
% \leq&2(2\rho - 1)\|Q_{ij}(t)\| + C_1 + C_2. \label{eq:norm-rel}
% \end{align}

% Clearly, if $\rho < \frac{1}{2}$, then there exists $\epsilon > 0$ and $B > 0$, when $L\big{(}Q(t)\big{)} > B$, we have,
% \[
% \mathbf{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\leq -\epsilon\|Q(t)\|.
% \]
% \end{IEEEproof}

% As mentioned in~\autoref{subsubsec:proof-technique},
% combine \autoref{lemma:qps-drift} and {\bf Theorem 2}
% in~\cite{Leonardi2001Stability},
% we can prove the stability
% of QPS-1. That is, QPS-1 can achieve at least $50\%$ and furthermore the queueing
% system is strongly stable when the maximum load factor $\rho < 0.5$. Note that
% {\bf Theorem 2} in~\cite{Leonardi2001Stability} proves that any queueing system
% satisfying the drift condition~\autoref{eq:qps-drift} is strongly stable, the proof
% of which is somehow standard and has been done in other literature.

% It is clear that the above proof can be directly applied to QPS-r, with $r>1$, since
% ~\eqref{eq:departure-row} and \eqref{eq:departure-column} are clearly
% satisfied by QPS-r, which are the only properties of QPS-1 used in the proof.

% % which
% % can be viewed as as a special case of Tweedy's Theorem in~\cite[Theorem C.4]{Gong2017QPS}.
% % Similar theorems are commonly used in the crossbar scheduling literature~\cite{McKeownMekkittikulAnantharamEtAl1999,Mekkittikul98stability}.


% %\begin{comment}
% % move to other part
% % \begin{theorem}{Stability of QPS}\label{thm:stability-qps}
% % If the maximum load factor $\rho < 0.5$, then the switched system applying QPS every time
% % slot is strongly stable.
% % \end{theorem}
% %\end{comment} 

==> sections/throughput_analysis_longbk_0729.tex <==
\section{Throughput and Delay Analysis}\label{sec:throughput-and-delay-analysis}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% This part of texts is an outline for this section
%% You can simply Line 16 of QPS.tex to noy include
%% this part.
\ifOutline
\fbox{\bf
\begin{minipage}[t]{0.45\textwidth}
\begin{center}{\color{red}$==========>$ outline $<===========$}\end{center}
\begin{enumerate}
\item Throughput analysis

A simple paragraph for the two commonly used proof techniques.

Prepare notations for Lyapunov function, then prove Lemma one followed by Theorem 1.

\item Delay analysis

A simple paragraph to describe Neely's proof. (summarize Neely's results in Theorem 2 \&
bring in the important property of maximal matching). Transit to QPS (from deterministic to
expectation). Prove the property of QPS and then discuss/explain their connections.

\end{enumerate}
\begin{center}
{\color{red}$======>$status: done $<========$}
\end{center}
\end{minipage}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% In this section, we prove that the QPS-r can achieve at least $50\%$
% throughput and derive its delay bounds. In~\autoref{subsec:background-notation},
% we introduce
% some background information and notations that we need in the stability proofs.
% In~\autoref{subsec:throughput-analysis}, we prove that QPS-r can achieve at least $50\%$
% throughput and derive its delay bounds in~\autoref{subsec: delay-analysis}.

% \subsection{Background and Notations}\label{subsec:background-notation}
\subsection{Preliminaries}\label{subsec:background-notation}\label{subsec:traffic-model}

% \subsubsection{Traffic Model}\label{subsec:traffic-model}

We first define three $N\times N$ matrices $Q(t)$, $A(t)$, and $D(t)$.
Let $Q(t) = \big{(}q_{ij}(t)\big{)}$ be the queue length matrix where $q_{ij}(t)$
is the length of the $j^{th}$ VOQ at input port $i$ during time slot $t$.
Let $A(t) = \big{(}a_{ij}(t)\big{)}$ be the traffic arrival matrix where $a_{ij}(t)$
is the number of packets arriving at the input port $i$ destined for
output port $j$ during time slot $t$.%, which can be viewed as the
counting process associated with underlying traffic arrival process.
Let $D(t) = \big{(}d_{ij}(t)\big{)}$ be the
departure matrix for time slot $t$ output by the crossbar scheduling algorithm.
Similar to $S(t)$, $D(t)$ is a $0$-$1$ matrix in which
$d_{ij}(t)=1$ if and only if there is a packet departing/transmitting
through VOQ$_{ij}$ during time slot $t$. Then, the queue length
matrix $Q$ evolves over time as follows.
\begin{equation}\label{eq:queueing-dynamics-entrywise}
q_{ij}(t + 1) = q_{ij}(t) - d_{ij}(t) + a_{ij}(t).
\end{equation}

Like in \cite{Gong2017QPS,Tassiulas90MaxWeight}, we assume that, for each $1\le i, j\le N$, $\{a_{ij}(t)\}_{t=0}^{\infty}$ is
a sequence of {\it i.i.d.} random variables,
%$i,j=1,2,\cdots,N$,
and the second moment
of their common distribution ($=\mathbb{E}\big{[}a^2_{ij}(0)\big{]}$) is finite.
% As mentioned above, our switch operates in slotted time, we assume that packets
% arrive at each input port can be modeled as a discrete-time Markov process. These discrete-time
% arrival processes can be characterized with an $N\times N$ matrix. Let $A(t)\!=\!\big{(}a_{ij}(t)\big{)}$
% denote this traffic arrival matrix in which $a_{ij}(t)$ is the amount of packets arriving to
% VOQ $j$ at the input port $i$ during time slot $t$.

Let $\lambda_{ij}$ be the normalized (to the percentage of the rate of an input/output link) mean arrival rate of packets to the $j^{th}$ VOQ (\ie those destined for
output port $j$) at input port $i$.  Then the
traffic pattern, can be represented by an $N \times N$ traffic matrix $\Lambda = \{\lambda_{ij}\}_{N\times N}$.
We also define $\rho$ as the maximum load factor imposed on any input or output port,
\begin{align}\label{def:lambda_max}
\rho \triangleq \max \big{\{} \max_{1\le i\le N}\{\lambda_i^{(in)}\}, \max_{1\le j\le N}\{\lambda_j^{(out)}\} \big{\}}
\end{align}
As mentioned before, we will prove %in~\autoref{sec:throughput-and-delay-analysis} 
in this section
that
QPS-r is stable and furthermore has good delay bound when the maximum load factor is less than half, i.e., 
$\rho < 1/2$.

\begin{comment}
We assume that, for any $1\leq i,j\leq N$,
$\big{\{}a_{ij}(\tau)\big{\}}_{\tau=1}^{\infty}$ is a sequence of independent and
identically distributed ({\it i.i.d.}) random variables of which the common distribution has
finite second moment, so that $\mathbb{E}\big{[}a^2_{ij}(t)\big{]}\!<\!\infty$ for any $t$.

Let $\lambda_{ij}=\mathbb{E}\big{[}a_{ij}(t)\big{]}$ be the average arrival rate to VOQ $j$ at input
port $i$. For ease of presentation in this paper, we define another $N\times N$ matrix, $\Lambda=\big{(}\lambda_{ij}\big{)}.
$We denote $\rho=\max\{\max_i \sum_j\lambda_{ij}, \max_j \sum_i \lambda_{ij}\}$ as the maximum load factor imposed on any input or output port. We will show later that
the switched system employing the QPS-r scheduling algorithm is stable (we will define it formally next)
whenever $\rho < 0.5$.

% \subsubsection{Queueing Dynamics}\label{subsec:queueing}

We define another two $N\times N$ matrices: $Q(t)$ and $S(t)$. Let $Q(t)\!=\!\big{(}q_{ij}(t)\big{)}$
be the queue length matrix in which $q_{ij}(t)$ denotes the number of packets
({\it i.e.,} VOQ length) buffered in VOQ $j$ at input port $i$ during time slot $t$. Similarly,
we denote $S(t)$ as the matching, or schedule during time slot $t$, that is, $s_{ij}(t)\!=\!1$ if
and only if input port $i$ matches with output port $j$ during time slot $i$, otherwise, $s_{ij}(t)=0$.
The queueing dynamics thus evolves as follows. For any $1\leq i,j\leq N$,
% \begin{equation}\label{eq:queueing-dynamics-entrywise-org}
% q_{ij}(t + 1) = \big{[}q_{ij}(t) + a_{ij}(t) - s_{ij}(t)\big{]}^{+}.
% \end{equation}
% remove (d(t)) dependency on a(t)
\begin{equation}\label{eq:queueing-dynamics-entrywise-org}
q_{ij}(t + 1) = \big{[}q_{ij}(t) - s_{ij}(t)\big{]}^{+} + a_{ij}(t) .
\end{equation}
where $[\cdot]^{+}\triangleq \max\{\cdot,0\}$.

For ease of analysis in this paper, we define another $N\times N$ $0$-$1$ matrix,
the departure matrix $D(t)=\big{(}d_{ij}(t)\big{)}$, in which $d_{ij}(t)$ is
the number of packets that is transmit from input port $i$ to output $j$. It is
clear that $d_{ij}=s_{ij}(t) \cdot 1_{\{q_{ij}(t) > 0\}}$ where
$1_{\{q_{ij}(t) > 0\}}$ is an indicator that equals $1$ if
$q_{ij}(t) > 0$ otherwise $0$. Therefore, the queueing dynamics equation
({\it i.e.,} \autoref{eq:queueing-dynamics-entrywise-org}) can be rewritten as,
\begin{equation}\label{eq:queueing-dynamics-entrywise}
q_{ij}(t + 1) = q_{ij}(t) - d_{ij}(t) + a_{ij}(t).
\end{equation}

\end{comment}
% \begin{definition}[Strongly Stable]\label{def:strongly-stable}
% A switched system with queue length matrix $\{Q(t)\}_{t=0}^{\infty}$ is {\bf strongly stable} if
% \[
% \lim\limits_{t\rightarrow \infty}\sup\mathbb{E}\big{[}\|Q(t)\|\big{]} < \infty,
% \]
% where $\|Q(t)\|=\sum_{i,j}q^2_{ij}(t)$.
% Note that this definition is the same as the one used
% in~\cite{Leonardi2001Stability}, which is slightly different from the one we used in our
% previous work~\cite{Gong2017QPS}. [equivalence]
% \end{definition}

\begin{comment}

\subsubsection{Proof Techniques}\label{subsubsec:proof-technique}

To show stability of a queueing system, there are two broad methods.
One is the fluid limit technique~\cite{Dai1995fluid}, and
the other is the Lyapunov function technique~\cite{Meyn2009BookMCSS}.
In this work, we are using the latter,
with which we construct a Lyapunov function, and
show that it has negative drift.
After that, we invoke {\bf Theorem 2} proved in~\cite{Leonardi2001Stability}, which
states that the queueing system is strongly stable if the negative drift
satisfies a stronger condition.

To further get the delay bounds of a queueing system, the general method is also
based on the Lyapunov function technique. One usually constructs a Lyapunov function,
which could be the same as or different than the one used in the stability proof.
And then analyze its unconditional drift, and by adding up infinite number of
such unconditional drift and using some Markov chain's properties,
the moment bound for the queue lengths is obtained.

[Prof. Siva maybe you can help me revise/add a few more high-level sentences on delay bound analysis
techniques]
\end{comment}

%%%%%%%% please move the proof of lemma 1 here
%%%%
%%%

\subsection{Throughput Analysis}\label{subsec:throughput-analysis}

In this subsection we prove that QPS-r can achieve at least $50\%$ throughput.
The following theorem summarize the main results of this section.

% \subsubsection{Main Results}\label{subsubsec: main-res}
% \begin{theorem}[Stability of QPS-r]\label{thm:stability-qps}
% When the maximum load factor $\rho<1/2$,
% the switching system scheduling according to QPS-r every time
% slot is stable in the following stability notion.
% The joint queueing and scheduling process $\{Q(t), S(t)\}_{t=0}^{\infty}$
% is an ergodic Markov chain, and as a consequence,
% the queueing process $\{Q(t)\}_{t=0}^{\infty}$
% converges in distribution to a random matrix $\hat{Q}=\big{(}\hat{q}_{ij}\big{)}$. Furthermore,
% \[
% \mathbb{E}\big{[}\|\hat{Q}\|_1\big{]} < \infty.
% \]
% where $\|\hat{Q}\|_1=\sum_{i,j}\hat{q}_{ij}$.
% \end{theorem}

% Note that the stability notion in the above theorem
% is commonly used in previous work ({\it e.g.,} \cite{McKeownMekkittikulAnantharamEtAl1999,Mekkittikul98stability,Gong2017QPS,Tassiulas1998,GiacconePrabhakarShah2003SERENA}). To prove~\autoref{thm:stability-qps}, we need to show
% that (I) the Markov chain is positive recurrent and hence converges to a stationary distribution, and
% (II) the stationary distribution has a finite first moment.
\begin{theorem}[Stability of QPS-r]\label{thm:stability-qps}
When the maximum load factor $\rho<1/2$,
the switching system scheduling according to QPS-r every time
slot is stable in the following notion:
The queueing process $\{Q(t)\}_{t=0}^{\infty}$
is a positive recurrent Markov chain.
\end{theorem}

By Foster-Lyapunov stability criterion~\cite[Proposition 2.1.1]{brucelecture2006}, to
prove the stability, we construct a Lyapunov function and obtain a negative drift
of it.
We accomplish the proof of the above theorem by analyzing the following Lyapunov function which was used in~\cite{Neely2008DelayMM, Neely2009MMDelay}, and is closely related to the Lyapunov function used in~\cite{Wu2007QueueGrouping,Dai00Speedup}.


% \begin{equation}\label{eq:lyapunov}
% L\big{(}Q(t)\big{)}=\sum_{i}Q_{i*}^2(t) + \sum_jQ_{*j}^2(t).
% \end{equation}
\begin{equation}\label{eq:lyapunov-org}
L\big{(}Q(t)\big{)}=\sum_{i,j}q_{ij}(t)\cdot\big{(}Q_{i*}(t) + Q_{*j}(t) - q_{ij}(t)\big{)}.
\end{equation}
where $Q_{i*}(t)$ and $Q_{*j}$ are the row sum of the $i^{th}$ row and
the column sum of the $j^{th}$
column of the queue length matrix $Q(t)$ respectively.
Mathematically, they are formally defined as follows.
\begin{align}
Q_{i*}(t)&=\sum_j q_{ij}(t) \label{eq:rowsum}\\
Q_{*j}(t)&=\sum_i q_{ij}(t). \label{eq:columnsum}
\end{align}
Note that this kind of notation applied to all other matrices defined in paper.
For example, $D_{i*}(t)$ denotes the row sum of the $i^{th}$ row of the departure
matrix $D(t)$.

For each VOQ$_{ij}$, we define its neighborhood as all the VOQs at its input and
at its output, including itself.
The total queue length at time slot $t$
of VOQs in the neighborhood is denoted $Q^\dagger_{ij}(t)$.
Clearly, $Q^\dagger_{ij}(t)=Q_{i*}(t) + Q_{*j}(t) - q_{ij}(t)$, hence the Lyapunov
function~\autoref{eq:lyapunov-org} can be re-written as,
\begin{equation}\label{eq:lyapunov}
L\big{(}Q(t)\big{)}=\sum_{i,j}q_{ij}(t)Q^\dagger_{ij}(t).
\end{equation}


Proof of Theorem 1 starts here -----------

Here we prove only the first part of the claim (that ... is positive recurrent), as the second part
(that ... < infinity) is implied by Theorem ?, which we will prove using some intermediate results
derived in this proof.   ...Q(t)... is clearly a Markov chain, since in (2), the term dijt is a function of 
Q(t) and aijt is a random variable independent of Q(t) 

To prove that ... is positive recurrent, it suffices to show that, there exists a constant $C > 0$ such that whenever $\|Q(t)\|_1 > C$, we have
\begin{equation}\label{eq:qps-drift}
\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon
\end{equation}
where $\epsilon > 0$ is a constant.  


\begin{comment}
relies on the drift condition
of $L\big{(}Q(t)\big{)}$ stated in the following lemma.
\begin{lemma}[Drift Under QPS]\label{lemma:qps-drift}
If QPS scheduling is applied in the input-queued switch every time slot, and the maximum load
factor $\rho < 0.5$, then there exist $B,\epsilon >0$ such that, when $L\big{(}Q(t)\big{)} > B$,
we have,
\begin{equation}\label{eq:qps-drift}
\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon\|Q(t)\|_2.
\end{equation}
where $\|Q(t)\|_2=\sqrt{\sum_{ij}q^2_{ij}(t)}$ is the L2 norm of $Q(t)$.
\end{lemma}
\end{comment}


\begin{comment}
%%%%%%%% moved to QPS-r property
To show the drift condition~\autoref{eq:qps-drift}, it relies on the following property of QPS-r.

\begin{lemma}[QPS-r Property]\label{lemma:QPS-property}
Under the QPS-r scheduling algorithm, for any time slot $t$, we have,
\begin{equation}\label{eq:QPS-property}
\sum_{i,j}\mathbb{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t)- q_{ij}(t)\big{]}\geq 0.
\end{equation}
\end{lemma}

We defer the proof of~\autoref{lemma:QPS-property} to~\autoref{subsubec:lemma-2-proof}.
Let us first recall the important property of
maximal matchings relating to it, which is commonly used in the previous work
({\it e.g.,} \cite{Neely2008DelayMM,Neely2009MMDelay,Dai00Speedup}) to analyze
the stability and delay bounds of queueing system scheduling according to maximal matchings.
That is $q_{ij}(t)D^{\dagger}_{ij}(t)- q_{ij}(t)\geq 0$, as $D^\dagger_{ij}(t)\geq 1$
when $q_{ij}(t)>0$ for maximal matchings. [A few sentences on the relation to be added.]

\end{comment}
\subsection{Proof of~\autoref{lemma:qps-drift}}\label{subsubsec:proof-lemma-1}
% In this section, we prove~\autoref{lemma:qps-drift}.

% \begin{IEEEproof}
\begin{comment}
By simple calculations and using~\eqref{eq:queueing-dynamics-entrywise}, we have,
\begin{align}
&L\big{(}Q(t+1)\big{)} \nonumber \\
=&\sum_{ij}q_{ij}(t+1)Q^\dagger_{ij}(t+1)\nonumber\\
=&\sum_{ij}\big{(}q_{ij}(t)+a_{ij}(t)-d_{ij}(t)\big{)}\big{(}Q^\dagger_{ij}(t)+A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\nonumber\\
=&\sum_{ij}q_{ij}(t)Q^\dagger_{ij}(t) + \sum_{ij}q_{ij}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+ \sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}Q^\dagger_{ij}(t) \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:ltplusone}
\end{align}

Focus on the third term on the right-hand-side (RHS) of~\autoref{eq:ltplusone}, we have,
\begin{equation*}
\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}Q^\dagger_{ij}(t)\!=\!\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)-\sum_{ij}d_{ij}(t)Q^\dagger_{ij}(t)
\end{equation*}

Focus on the first term on the RHS of the above equation, we have,
\begin{align}
&\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)\nonumber\\
=&\sum_{ij}a_{ij}(t)\big{(}Q_{i*}(t)+Q_{*j}(t)-q_{ij}(t)\big{)}\nonumber\\
=&\sum_{ij}a_{ij}(t)Q_{i*}(t)\! +\! \sum_{ij}a_{ij}(t)Q_{*j}(t)\!-\!\sum_{ij}a_{ij}(t)q_{ij}(t)\label{eq:term-01}
\end{align}
Continue focusing the the first term on the RHS of the above equation, we have
\begin{align}
\sum_{ij}a_{ij}(t)Q_{i*}(t)&=\sum_{i}\big{(}Q_{i*}(t)\sum_{j}a_{ij}(t)\big{)}\nonumber\\
&=\sum_{i}Q_{i*}(t)A_{i*}(t)\nonumber\\
&=\sum_{i}\big{(}\sum_{j}q_{ij}(t)\big{)}A_{i*}(t)\nonumber\\
&=\sum_{ij}q_{ij}(t)A_{i*}(t)\label{eq:tterm-01}
\end{align}

Similarly, for the second term, we have,
\begin{equation}\label{eq:tterm-02}
\sum_{ij}a_{ij}(t)Q_{*j}(t)=\sum_{ij}q_{ij}(t)A_{*j}(t).
\end{equation}

Substitute \autoref{eq:tterm-01} and \autoref{eq:tterm-02} into \autoref{eq:term-01}, we have,
\begin{equation}\label{eq:term-a}
\sum_{ij}a_{ij}(t)Q^\dagger_{ij}(t)=\sum_{ij}q_{ij}(t)A^\dagger_{ij}(t)
\end{equation}

Similarly, we have,
\begin{equation}\label{eq:term-d}
\sum_{ij}d_{ij}(t)Q^\dagger_{ij}(t)=\sum_{ij}q_{ij}(t)D^\dagger_{ij}(t)
\end{equation}

Substitute \autoref{eq:term-a} and \autoref{eq:term-d} into the third term on
the right-hand-side (RHS) of~\autoref{eq:ltplusone}, we have,
\begin{align}
&L\big{(}Q(t+1)\big{)}\nonumber\\
=&\sum_{ij}q_{ij}(t)Q^\dagger_{ij}(t) + 2\sum_{ij}q_{ij}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\nonumber\\
=&L\big{(}Q(t)\big{)}+ 2\sum_{ij}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:derived-drift}
\end{align}

Thus,
\end{comment}




%
It is not hard to check (for more detailed steps, please refer to~\cite{Neely2008DelayMM}),
\begin{align}
&L\big{(}Q(t+1)\big{)}-L\big{(}Q(t)\big{)}\nonumber\\
=&2\sum_{ij}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}  \nonumber\\
&+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\label{eq:uncond-drift}
\end{align}

Hence the drift of the Lyapunov function~\autoref{eq:lyapunov} can written as,
\begin{align}
&\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\nonumber\\
=&\mathbb{E}\Big{[}2\sum_{ij}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} \nonumber\\
&\mathbb{E}\Big{[}+\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} \label{eq:raw-drift}
\end{align}

[to be moved further down]
Note that the LHS of ... and the LHS ... are the first term and the second term respectively in ... before the expectations are taken.  


To prove the negative drift of the Lyapunov function~\autoref{eq:lyapunov}, we will show that
the first term on the RHS of~\autoref{eq:raw-drift} is bounded by $2(2\rho-1)\|Q(t)\|_1$, and
the second one can be bounded by a constant for any fixed $N$. More formally, we will prove the
following two inequalities.


Now we claim following two inequalities, which we will prove shortly.
\begin{eqnarray}
\sum_{ij}\mathbb{E}\big{[}q_{ij}(t)\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\big{]}\!\leq\! (2\rho \!-\! 1)\|Q(t)\|_1\label{eq:term-1-tbp}\\
\sum_{ij}\mathbb{E}\big{[}\big{(}a_{ij}(t)\!-\!d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\big{]} \!\leq\! the detailed term \label{eq:term-2-tbp}
\end{eqnarray}

With ... and ..., we have 
$... < (2\rho \!-\! 1)\|Q(t)\|_1 + the detailed term$.  

%CN^2,
where $C > 0$ is a constant.

First, let us focus on the proof of~\autoref{eq:term-1-tbp}, which is
a simple derivation based on~\autoref{lemma:QPS-property}, although
we will show later that the proof of~\autoref{lemma:QPS-property} is
quite involved, which we consider as one major contribution of this work.
Using the results of~\autoref{lemma:QPS-property}, we have,
\begin{align}
&\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\Big{]}\nonumber\\
=&\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)A^\dagger_{ij}(t) \Big{]}-\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)D^\dagger_{ij}(t)\Big{]}\nonumber\\
\leq&\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)A^\dagger_{ij}(t) \Big{]}-\sum_{ij}\mathbb{E}[q_{ij}(t)]\nonumber\\
=&\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)(A^\dagger_{ij}(t)-1)\Big{]}. \label{eq:bounded-first-term}
\end{align}

Now we proceed to prove~\autoref{eq:term-2-tbp}, similar proof can
be found in~\cite{Neely2008DelayMM}.
As $a_{ij}(t)$ is {\it i.i.d.} for any $i,j=1,2,\cdots,N$ (assumed in~\autoref{subsec:traffic-model}), we have,
\begin{align}
&\mathbb{E}\big{[}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\big{]}\nonumber\\
=&\mathbb{E}[a_{ij}(t)A^\dagger_{ij}(t) - d_{ij}(t)A^\dagger_{ij}(t)-a_{ij}(t)D^\dagger_{ij}(t)+d_{ij}(t)D^\dagger_{ij}(t)]\nonumber\\
=&\mathbb{E}[a^2_{ij}(t)]\!-\!\lambda^2_{ij}\!+\!\lambda_{ij}\Lambda^{\dagger}_{ij}
\!-\!\mathbb{E}[d_{ij}(t)]\Lambda^\dagger_{ij} \nonumber\\
&-\lambda_{ij}(t)\mathbb{E}[D^\dagger_{ij}(t)]\!+\! \mathbb{E}[d_{ij}(t)D^\dagger_{ij}(t)]\nonumber\\
=&\mathbb{E}[a^2_{ij}(t)]\!-\!\lambda^2_{ij}\!+\!\lambda_{ij}\Lambda^{\dagger}_{ij}
\!-\!\mathbb{E}[d_{ij}(t)]\Lambda^\dagger_{ij} \nonumber\\
&-\lambda_{ij}(t)\mathbb{E}[D^\dagger_{ij}(t)]\!+\! \mathbb{E}[d_{ij}(t)]. \label{eq:bt}
\end{align}

In the last step of the above derivation, we use the following fact of $D(t)$:
for any $i,j=1,2,\cdots,N$ we have $d_{ij}(t)D^\dagger_{ij}(t)= d_{ij}(t)$.
Because $d_{ij}(t)\in\{0,1\}$, and $D^\dagger_{ij}(t)= 1$ if $d_{ij}(t)=1$, otherwise $d_{ij}(t)D^\dagger_{ij}(t)=0=d_{ij}(t)$.

Recall (from~\autoref{subsec:traffic-model}) that $\mathbb{E}[a^2_{ij}(t)]<\infty$ (our assumption).
Besides $d_{ij}(t)\leq 1$, $D^\dagger_{ij}(t)\leq2$, $\lambda_{ij}\leq\rho<1/2$, and $\Lambda^\dagger_{ij}\leq 2\rho<1$, for all $i,j=1,2,\cdots,N$, hence there exist some constant $C>0$ such that,
\begin{equation*}
\mathbb{E}\Big{[}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]} < C.
\end{equation*}

Therefore, for a fixed $N$, the second term of~\autoref{eq:raw-drift} is bounded,
\begin{equation}\label{eq:bounded-term}
\sum_{ij}\mathbb{E}\Big{[}\big{(}a_{ij}(t)\!-\!d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)\!-\!D^\dagger_{ij}(t)\big{)}\mid Q(t)\Big{]}\!\leq\! CN^2.
\end{equation}


Now we can obtain the negative drift of~\autoref{lemma:qps-drift} by simply substituting~\autoref{eq:bounded-term} and \autoref{eq:bounded-first-term} into~\autoref{eq:raw-drift}.
\begin{align*}
&\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\nonumber\\
% \leq&2\sum_{ij}\mathbb{E}\Big{[}q_{ij}(t)(A^\dagger_{ij}(t)-1) \mid Q(t)\Big{]} + CN^2\nonumber\\
\leq&2(2\rho-1)\|Q(t)\|_1 + CN^2 \nonumber\\
=&-2(1 - 2\rho)\|Q(t)\|_1 + CN^2 \nonumber\\
\leq&-2(1 - 2\rho)\|Q(t)\|_2 + CN^2.
\end{align*}
In the last step we use the following well-known mathematical fact: for any finite dimension
vector $X$, we have $\|X\|_1\geq \|X\|_2$.

Therefore, we have, there exist $B,\epsilon >0$ such that, when $L\big{(}Q(t)\big{)} > B$,
\begin{equation*}
\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \leq -\epsilon\|Q(t)\|_2.
\end{equation*}

% \end{IEEEproof}
\noindent
{\bf Remarks.} The drift condition we obtained in the proof of~\autoref{lemma:qps-drift}
is stronger than the requirement of the Foster-Lyapunov stability
criterion~\cite[Proposition 2.1.1]{brucelecture2006}, which
only requires the drift
$\!\leq\! -\epsilon$ for some $\epsilon>0$ when $L\big{(}Q(t)\big{)} \!>\! B$.
With this stronger drift condition and using similar
approaches as in~\cite{Gong2017QPS,Tassiulas1998},
we can prove a stronger stability notion --
the first moment of the stationary distribution is bounded, {\it i.e.,}
$\|\hat{Q}\|_1\!<\!\infty$, where $\hat{Q}$ is the random matrix the
queueing process $\{Q(t)\}_{t=0}^{\infty}$ converges to in distribution.
Here, we skip the proof,
because we will prove next a even
stronger result -- the first moment of the stationary distribution
is bounded by some
constants for fixed $N$, furthermore the bound is $\frac{1}{1-2\rho}$
for Bernoulli {\it i.i.d.} traffic.

\subsection{Proof of \autoref{lemma:QPS-property}}\label{subsubec:lemma-2-proof}
In this section, we prove~\autoref{lemma:QPS-property}.
First, we analyze $\mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}$.
From the queue proportional sampling proposing strategy
described in~\autoref{subsubsec:qps-proposing}, we have, under
QPS-1, for any $i$,
\begin{equation}\label{eq:departure-row-org}
\mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
\end{equation}
where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
VOQ $j$ in the proposing stage. Clearly, we have, under QPS-1, for any $i,j$,
\begin{equation}\label{eq:cond-accept-p}
\alpha_{ij}(t)=\mathbb{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
\end{equation}

According to the description of QPS-r in~\autoref{subsec:qps-r}, we have, we have, under
QPS-r, for any $i$,
\begin{equation}\label{eq:departure-row}
\mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}\geq\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
\end{equation}

Similarly, we have, under QPS-r, for any $j$,
\begin{equation}\label{eq:departure-column}
\mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}\geq1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
\end{equation}
It is clear that the second term above is the probability that no input port
proposes to output port $j$. It is the only case that $D_{*j}(t)=0$, because
each input port proposes only when the corresponding VOQ is not empty and
according to the accepting strategy described
in~\autoref{subsubsec:qps-accepting}, as long as
there are proposal(s) output port $j$ would accept one (no matter which one).

Now we proceed to prove \autoref{lemma:QPS-property}.
\begin{IEEEproof}
It suffices to show that for any $i$ and $j$, we have 
\begin{equation}
\sum_{i,j}\mathbb{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]} \ge \sum_{i,j}q_{ij}(t) (label it)
\end{equation}
because with (label it), we have
\begin{equation}
\sum_{i,j}\mathbb{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t)\big{]}\!=\!\mathbb{E}\Big{[}\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\Big{]}.
\end{equation}
$\ge \mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)\big{]} = \sum_{i,j}\mathbb{E}\big{[}q_{ij}(t)\big{]} (Long, shift it to the right place)$
% Then, from the definition of $\hat{D}_{ij}(t)$, for any $i,j=1,2,\cdots,N$, we have,
% \begin{equation}\label{eq:group-depart}
% \hat{D}_{ij}(t)=D_{i*}(t) + D_{*j}(t) - d_{ij}(t).
% \end{equation}

From the definition of $D^{\dagger}_{ij}(t)$, we have,
\begin{align}
&\sum_{,j}q_{ij}(t)D^{\dagger}_{ij}(t) \nonumber \\
=&\sum_{i,j}q_{ij}(t)\big{(}D_{i*}(t) - d_{ij}(t) + D_{*j}(t)\big{)} \nonumber \\
=&\sum_{i}Q_{i*}(t)D_{i*}(t) \!-\!\sum_{i,j}q_{ij}(t)d_{ij}(t) \!+\! \sum_{j}Q_{*j}(t)D_{*j}(t) \nonumber
\end{align}

By simple calculations and using~\eqref{eq:departure-row} and \eqref{eq:departure-column},
we have,

\begin{align}
&\sum_{i,j} \mathbb{E}\big{[}q_{ij}(t)D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\nonumber \\
=&\sum_{i,j} q_{ij}(t)\mathbb{E}\big{[}D^{\dagger}_{ij}(t) \mid Q(t)\big{]}\nonumber \\
=&\sum_{i,j} q_{ij}(t)\mathbb{E}\big{[}D_{i*}(t) - d_{ij}(t) + D_{*j}(t)  \mid Q(t)\big{]}\nonumber \\
=& summaton-of-three-conditional-expectations \nonumber \\
=&\sum_{i}Q_{i*}(t)\mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]} \!-\!\sum_{i,j} q_{ij}(t) \mathbb{E}\big{[}d_{ij}(t)\mid Q(t)\big{]} \!+\! \sum_{j} Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]} \nonumber\\
\geq&\sum_{i,j}q_{ij}(t)\alpha_{ij}(t) - \sum_{i,j}q_{ij}(t)\mathbb{E}\big{[}d_{ij}(t) \mid Q(t)\big{]}\nonumber\\
&+ \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{i,j}q_{ij}(t)\alpha_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)} + \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
\geq&\sum_{i,j}q_{ij}(t)\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}\prod_{k\neq i}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\nonumber\\
&+ \sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{i,j}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}+\sum_{j=1}^{N}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
\geq&\sum_{j}Q_{*j}(t)\Big{(}1 \!-\! \mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
&\!+\!\sum_{j}Q_{*j}(t)\mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]} \nonumber\\
=&\sum_{j}Q_{*j}(t)=\sum_{i,j}q_{ij}(t)=\mathbb{E}\big{[}\sum_{i,j}q_{ij}(t)\mid Q(t)\big{]}. \nonumber
\end{align}

Therefore, we have property~\autoref{eq:QPS-property} holds.
\end{IEEEproof}

% We first analyze the drift of the first term of the Lyapunov function~\eqref{eq:lyapunov}.
% By simple calculations and using~\eqref{eq:queueing-dynamics-entrywise}, we have,
% \begin{align}
% &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&\mathbb{E}\Big{[}\sum_i \big{(}A_{i*}(t) \!-\! D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) \!+\! A_{i*}(t) \!-\! D_{i*}(t)\big{)}
% \mid Q(t) \Big{]}\nonumber
% \end{align}

% Use the linearity of expectation and the fact that
% $\mathbb{E}\big{[}A_{i*}(t)\big{]}=\Lambda_{i*}$ for any $i$ and $t$, we have,
% \begin{align}
% &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\nonumber\\
% =&2\sum_{i}Q_{i*}(t)\Big{(}\Lambda_{i*} - \mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% &+ \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:first-term-using-avg-departure}
% \end{align}

% Let analyze the term $\mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}$ in the first term above.
% From the queue proportional sampling proposing strategy
% described in~\autoref{subsubsec:qps-proposing}, we have, for any $i$,
% \begin{equation}\label{eq:departure-row}
% \mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
% \end{equation}
% where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
% input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
% event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
% VOQ $j$ in the proposing stage. Clearly, we have, for any $i,j$,
% \begin{equation}\label{eq:cond-accept-p}
% \alpha_{ij}(t)=\mathbb{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
% \end{equation}

% % Similarly, we have, for any $j$,
% % \begin{equation}\label{eq:departure-column}
% % \mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% % \end{equation}

% Substitute~\autoref{eq:cond-accept-p} and \autoref{eq:departure-row}
% into \autoref{eq:first-term-using-avg-departure}, we have,
% \begin{align}
% &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&2\sum_{i}Q_{i*}(t)\Big{(}\Lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t)\Big{)} \nonumber\\
% &+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\nonumber\\
% =&2\sum_{i}\Lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \alpha_{ij}(t)\big{)}\nonumber\\
% &+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% \end{align}

% % From \autoref{eq:queueing-dynamics-entrywise}, we have, for any $i$,
% % \begin{equation}\label{eq:queue-dynamics-row}
% % Q_{i*}(t+1)=Q_{i*}(t) + A_{i*}(t) - D_{i*}(t),
% % \end{equation}
% % and for any $j$,
% % \begin{equation}\label{eq:queue-dynamics-column}
% % Q_{*j}(t+1)=Q_{*j}(t) + A_{*j}(t) - D_{*j}(t).
% % \end{equation}

% % By the description of the QPS policy in~\autoref{subsec:QPS},
% % From the queue proportional sampling proposing strategy
% % described in~\autoref{subsubsec:qps-proposing}, we have, for any $i$,
% % \begin{equation}\label{eq:departure-row}
% % \mathbb{E}\big{[}D_{i*}(t) \mid Q(t)\big{]}=\sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \alpha_{ij}(t),
% % \end{equation}
% % where $\alpha_{ij}(t)$ is a conditional probability of the event that the proposal from
% % input port $i$ is accepted by output port $j$ during time slot $t$, conditioning on the
% % event that input port $i$ does propose to output port $j$, that is, input port $i$ picks
% % VOQ $j$ in the proposing stage. Clearly, we have, for any $i,j$,
% % \begin{equation}\label{eq:cond-accept-p}
% % \alpha_{ij}(t)=\mathbb{E}\big{[}d_{ij}(t)\mid Q(t)\big{]}\Big{(}\frac{q_{ij}(t)}{Q_{i*}(t)}\Big{)}^{-1}.
% % \end{equation}

% % Similarly, we have, for any $j$,
% % \begin{equation}\label{eq:departure-column}
% % \mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% % \end{equation}

% % After all the above preparations, we can proceed to analyze the drift of the Lyapunov function
% % ~\autoref{eq:lyapunov}. Let us first deal with the drift of its first term,
% % {\it i.e.,} $\sum_i Q^2_{i*}(t)$.

% % \begin{widetext}
% % \begin{align}
% % &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) - \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&\mathbb{E}\Big{[}\sum_i \big{(}A_{i*}(t) - D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) + A_{i*}(t) - D_{i*}(t)\big{)}
% % \mid Q(t) \Big{]} \label{eq:using-queue-dynamics}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} + \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:using-arrival}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \hat{p}_{ij}(t)\Big{)} + \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-depature}\\
% % =&2\sum_{i}\lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \hat{p}_{ij}(t)\big{)}+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% % \end{align}
% % \end{widetext}
% % \begin{align}
% % &\mathbb{E}\big{[}\sum_{i}Q_{i*}^2(t+1) \!-\! \sum_{i}Q_{i*}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&\mathbb{E}\Big{[}\sum_i \big{(}A_{i*}(t) \!-\! D_{i*}(t)\big{)}\big{(}2Q_{i*}(t) \!+\! A_{i*}(t) \!-\! D_{i*}(t)\big{)}
% % \mid Q(t) \Big{]} \label{eq:using-queue-dynamics}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \mathbb{E}\big{[}D_{i*}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% % &+ \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]} \label{eq:using-arrival}\\
% % =&2\sum_{i}Q_{i*}(t)\Big{(}\lambda_{i*} - \sum_{j}\frac{q_{ij}(t)}{Q_{i*}(t)}\cdot \hat{p}_{ij}(t)\Big{)} \nonumber\\
% % &+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-depature}\\
% % =&2\sum_{i}\lambda_{i*}Q_{i*}(t) - 2\sum_{i}\sum_{j}\big{(}q_{ij}(t)\cdot \hat{p}_{ij}(t)\big{)}\nonumber\\
% % &+ \sum_i \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}. \label{eq:drift-term-1}
% % \end{align}

% % \noindent
% % \textbf{Remarks}. {\it 1)} Equality in \autoref{eq:using-queue-dynamics} is due to the queueing dynamics in~\autoref{eq:queue-dynamics-row}. {\it 2)} Equality in \autoref{eq:using-arrival} uses the linearity of expectation and the fact that
% % $\mathbb{E}\big{[}A_{i*}(t)\big{]}=\lambda_{i*}$ for any $i$ and $t$. {\it 3)} Equality in \autoref{eq:using-depature} is because of~\autoref{eq:departure-row}. {\it 4)} To avoid discussing the cases of ``dividing by zero'', we use the convention that $0/0=0$ in this
% % proof.

% Similarly, for the second term in the Lyapunov function~\eqref{eq:lyapunov}, we have,
% % \begin{table*}[!htb]
% % \centering
% % \begin{minipage}{0.8\textwidth}

% % \begin{widetext}
% % \begin{align}
% % % &\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% % % =&2\sum_{j}(\lambda_{*j} - 1) Q_{*j} + \sum_j \Big{(}Q_{*j}\prod_{i}\big{(}1 - \frac{Q_{ij}(t)}{Q_{i*}(t)}\big{)}\Big{)} \nonumber \\
% % % &+ \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}
% % &\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% % =&2\sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) + \sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % + \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:drift-term-2}
% % \end{align}
% % \end{widetext}
% % \end{minipage}
% % \end{table*}
% \begin{align}
% &\mathbb{E}\big{[}\sum_{j}Q_{*j}^2(t+1) - \sum_{j}Q_{*j}^2(t) \mid Q(t) \big{]} \nonumber\\
% =&2\sum_{j}Q_{*j}(t)\Big{(}\Lambda_{*j} - \mathbb{E}\big{[}D_{*j}(t)\mid Q(t)\big{]}\Big{)} \nonumber\\
% &+ \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:using-column-departure}\\
% =&2\sum_{j}(\Lambda_{*j} - 1) Q_{*j}(t) + \sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} \nonumber\\
% &+ \sum_j \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\label{eq:drift-term-2}
% \end{align}

% In the above derivation from \autoref{eq:using-column-departure} to \autoref{eq:drift-term-2},
% we use the following
% property of the column sum, $D_{*j}(t)$, of the departure matrix $D(t)$.
% \begin{equation}\label{eq:departure-column}
% \mathbb{E}\big{[}D_{*j}(t) \mid Q(t)\big{]}=1 - \prod_{i}\big{(}1 - \frac{q_{ij}(t)}{Q_{i*}(t)}\big{)}.
% \end{equation}
% It is clear that the second term above is the probability that no input port
% proposes to output port $j$. It is the only case that $D_{*j}(t)=0$, because
% each input port proposes only when the corresponding VOQ is not empty and
% according to the accepting strategy described
% in~\autoref{subsubsec:qps-accepting}, as long as
% there are proposal(s) output port $j$ would accept one (no matter which one).

% Now we proceed to analyze~\autoref{eq:drift-term-1}. Because,
% \[
% |A_{i*}(t) - D_{i*}(t)| \leq A_{i*}(t) + 1.
% \]
% and our assumption that each element of the arrival process $A(t)$ have
% a finite second moment in~\autoref{subsec:traffic-model},
% we have, there exists some constant $C_1$ such that for any $i$,
% \begin{equation}\label{eq:bounded-moment-row}
% \mathbb{E}\Big{[}\big{(}A_{i*}(t) - D_{i*}(t)\big{)}^2 \mid Q(t) \Big{]}\leq \mathbb{E}\Big{[}\big{(}A_{i*}(t) \!+\! 1\big{)}^2 \Big{]}\!\leq\! \frac{C_1}{N}.
% \end{equation}
% Similarly, we have there exists some constant $C_2$ such that for any $j$,
% \begin{equation}\label{eq:bounded-moment-column}
% \mathbb{E}\Big{[}\big{(}A_{*j}(t) - D_{*j}(t)\big{)}^2 \mid Q(t) \Big{]}\leq \frac{C_2}{N}.
% \end{equation}

% Now, we do some relaxation on $\alpha_{ij}(t)$, which is the probability that the proposal from
% input port $i$ is accepted by output port $j$ conditioning on that input port $i$ does propose
% to output port $j$. It is obvious that the proposal from input port $i$ {\bf has to} be accepted
% if it is the only proposal that output port $j$ receives. Therefore, we have, for any $i,j$,
% \begin{equation}\label{eq:accepting-prob}
% \alpha_{ij}(t)\geq \prod_{k\neq i} \big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)} \geq \prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}.
% \end{equation}

% Combining \autoref{eq:drift-term-1}, \autoref{eq:drift-term-2}, \autoref{eq:bounded-moment-row}, \autoref{eq:bounded-moment-column}, and \autoref{eq:accepting-prob}, we have,

% % \begin{widetext}
% % \begin{align}
% % &\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \nonumber \\
% % \leq&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)
% % -\sum_{i,j} \Big{(}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % +\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber\\
% % =&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)
% % -\sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}
% % +\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber \\
% % =&2\Big{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\Big{)} + C_1 +C_2 \nonumber \\
% % \leq&2(2\rho - 1)\|Q_{ij}(t)\|_1 + C_1 + C_2 \label{eq:arrival-adm}\\
% % \leq&2(2\rho - 1)\|Q_{ij}(t)\| + C_1 + C_2. \label{eq:norm-rel}
% % \end{align}
% % \end{widetext}

% \begin{align}
% &\mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]} \nonumber \\
% \leq&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\nonumber\\
% &-\sum_{i,j} \Big{(}q_{ij}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)} \nonumber\\
% &+\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber\\
% =&2\Bigg{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t) \nonumber\\
% &-\sum_j \Big{(}Q_{*j}(t)\prod_{k}\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\nonumber\\
% &+\sum_{j}\Big{(}Q_{*j}(t) \prod_k\big{(}1 - \frac{q_{kj}(t)}{Q_{k*}(t)}\big{)}\Big{)}\Bigg{)} + C_1 + C_2 \nonumber \\
% =&2\Big{(}\sum_{i}\lambda_{i*}Q_{i*}(t) + \sum_{j}(\lambda_{*j} - 1) Q_{*j}(t)\Big{)} + C_1 +C_2 \nonumber \\
% \leq&2(2\rho - 1)\|Q_{ij}(t)\|_1 + C_1 + C_2 \label{eq:arrival-adm}\\
% \leq&2(2\rho - 1)\|Q_{ij}(t)\| + C_1 + C_2. \label{eq:norm-rel}
% \end{align}

% Clearly, if $\rho < \frac{1}{2}$, then there exists $\epsilon > 0$ and $B > 0$, when $L\big{(}Q(t)\big{)} > B$, we have,
% \[
% \mathbb{E}\big{[}L\big{(}Q(t+1)\big{)} - L\big{(}Q(t)\big{)} \mid Q(t)\big{]}\leq -\epsilon\|Q(t)\|.
% \]
% \end{IEEEproof}

% As mentioned in~\autoref{subsubsec:proof-technique},
% combine \autoref{lemma:qps-drift} and {\bf Theorem 2}
% in~\cite{Leonardi2001Stability},
% we can prove the stability
% of QPS-1. That is, QPS-1 can achieve at least $50\%$ and furthermore the queueing
% system is strongly stable when the maximum load factor $\rho < 0.5$. Note that
% {\bf Theorem 2} in~\cite{Leonardi2001Stability} proves that any queueing system
% satisfying the drift condition~\autoref{eq:qps-drift} is strongly stable, the proof
% of which is somehow standard and has been done in other literature.

% It is clear that the above proof can be directly applied to QPS-r, with $r>1$, since
% ~\eqref{eq:departure-row} and \eqref{eq:departure-column} are clearly
% satisfied by QPS-r, which are the only properties of QPS-1 used in the proof.

% % which
% % can be viewed as as a special case of Tweedy's Theorem in~\cite[Theorem C.4]{Gong2017QPS}.
% % Similar theorems are commonly used in the crossbar scheduling literature~\cite{McKeownMekkittikulAnantharamEtAl1999,Mekkittikul98stability}.


% %\begin{comment}
% % move to other part
% % \begin{theorem}{Stability of QPS}\label{thm:stability-qps}
% % If the maximum load factor $\rho < 0.5$, then the switched system applying QPS every time
% % slot is strongly stable.
% % \end{theorem}
% %\end{comment} 

==> sections/throughput_delay_analysis_delay_analysis.tex <==
\subsection{Delay Analysis}\label{subsec: delay-analysis}

In this section, we derive the queue length bound (readily convertible to the delay
bound by Little's Law) for QPS-1 under {\it i.i.d.} traffic arrivals using
%. To prove the delay bound of QPS-r, we need
the following moment bound theorem~\cite[Proposition 2.1.4]{brucelecture2006}.
This bound, shown in~\autoref{eq:final-delay-bound}, is identical to that derived in~\cite[Section III.B]{Neely2008DelayMM,Neely2009MMDelay} for maximal matchings
under {\it i.i.d.} traffic arrivals.  Note this equivalence is not limited to {\it i.i.d.} traffic arrivals:
It can be shown that the
delay analysis results for general Markovian arrivals derived in~\cite{Neely2008DelayMM,Neely2009MMDelay} for maximal
matchings (using the stronger ``departure inequality''~\autoref{eq:QPS-property-strong}) hold also for QPS-1.

%Although in the interest of space, in this work we only show the delay analysis for the {\it i.i.d.} traffic arrivals,
%those for more general arrivals are almost
%identical. 
%The generalization is significant because ... }
%{\bf Prof. Siva: Maybe you can help add the following words.}


% stated as follows.
%[Moment bound~\cite{brucelecture2006}]

\begin{theorem}\label{thm:moment-bound}
Suppose that $\{Y_t\}_{t=0}^{\infty}$ is a positive recurrent Markov chain with countable state space $\mathcal{Y}$. Suppose $V$, $f$, and $g$ are non-negative functions on $\mathcal{Y}$ such that,
\begin{equation}\label{eq:mbreq}
V(Y_{t+1}) -V(Y_{t})\leq -f(Y_{t}) + g(Y_{t}), \,\mbox{for all } Y_{t} \in \mathcal{Y}
\end{equation}
% Then $\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[f(Y_t)]\!\leq\! \lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[g(Y_t)]$.
%% carry out Prof. Siva's comments @05/14/2019
Then $\mathbf{E}[f(\bar{Y})]\!\leq\! \mathbf{E}[g(\bar{Y})]$, where $\bar{Y}$ is a random variable with the stationary 
distribution of the Markov chain $\{Y_t\}_{t=0}^\infty$.
\end{theorem}

Now we derive the queue length bound for QPS-1 when the maximum load factor $\rho\!<\!1/2$. The queue length bound is formally stated in 
the following theorem. 
\begin{theorem}
Given a switching system under QPS-1, whenever the maximum load factor $\rho<1/2$, the steady state mean queue length is 
bounded. More precisely, we have,
\begin{equation}\label{eq:final-delay-bound}
\mathbf{E}[\|\bar{Q}\|_1]\leq\frac{1}{2(1-2\rho)}\sum_{i,j}\big{(}\sigma^2_{ij}\!-\!\lambda_{ij}\Lambda^\dagger_{ij}\!+\!\lambda_{ij}\big{)}.
\end{equation}
\end{theorem}
\begin{proof}
We define $V$, $Y_t$, $f$, and $g$ terms in %this theorem 
\autoref{thm:moment-bound} in such a way that the LHS and the RHS of \autoref{eq:mbreq}
become the LHS and the RHS of~\autoref{eq:uncond-drift} respectively (e.g., define $V$ as $L$, $Y_t$ as $Q(t)$, and $f(Y_t)$ as $-2\sum_{i,j}q_{ij}(t)\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}$).
%Let $Y_t\!=\!Q(t)$, then Then $Y_t$ is a positive recurrent Markov chain (proved in~\autoref{subsec:throughput-analysis}). Let $V(Y_t)$ be $L(Q(t))$ defined in~\autoref{subsec:throughput-analysis}, $-%f(Y_t)$ and $g(Y_t)$ be the first term and the second term on the RHS of~\autoref{eq:uncond-drift} respectively.
Then, we have,
% \begin{align}
% &\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}-2(2\rho-1)\mathbf{E}[\|Q(t)\|_1]\nonumber\\
% \leq&\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[f(Y_t)]\label{eq:qb-explain-01}\\
% \leq&\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[g(Y_t)]\label{eq:qb-explain-02}\\
% =&\sum_{i,j}\big{(}\sigma^2_{ij}\!-\!\lambda_{ij}\Lambda^\dagger_{ij} +\lambda_{ij}\big{)}.\label{eq:qb-explain-03}
% \end{align}
%% carry out Prof. Siva's comments
\begin{align}
&-2(2\rho-1)\mathbf{E}[\|\bar{Q}\|_1]\nonumber\\
\leq&\mathbf{E}[f(\bar{Y})]\label{eq:qb-explain-01}\\
\leq&\mathbf{E}[g(\bar{Y})]\label{eq:qb-explain-02}\\
=&\sum_{i,j}\big{(}\sigma^2_{ij}\!-\!\lambda_{ij}\Lambda^\dagger_{ij} +\lambda_{ij}\big{)}.\label{eq:qb-explain-03}
\end{align}
In the above derivation, inequality \autoref{eq:qb-explain-01} is
due to~\autoref{eq:term-1-tbp} (whose LHS is $-f(Y_{t})$), inequality \autoref{eq:qb-explain-02} is
due to~\autoref{thm:moment-bound}, and equality~\autoref{eq:qb-explain-03} is
due to~\autoref{eq:for-delay-analysis}.
% (when the $\sum_{i,j}$ operator is applied to both sides of it).


%Note that
%the derivation from \autoref{eq:term-2-tbp}
%to inequality \autoref{eq:qb-explain-01} requires a few trivial steps, which
%are omitted in the interest of space.


\begin{comment}
\begin{corollary}
For queueing system scheduling according to QPS-r, if the maximum load factor $\rho<1/2$, then
the total average queue length satisfies,
\begin{eqnarray}\label{eq:queue-length-bound}
\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[\|Q(t)\|_1] \!\leq\! \frac{1}{2(1\!-\!2\rho)}\sum_{i,j}\big{(}\sigma^2_{ij}\!-\!\lambda_{ij}\Lambda^\dagger_{ij} +\lambda_{ij}\big{)}.
\end{eqnarray}
where $\sigma^2_{ij}=\mathbf{E}[a^2_{ij}(t)]-\lambda^2_{ij}$ is the variance of $a_{ij}(t)$.
\end{corollary}
\begin{IEEEproof}
Note that, the proof is almost the same as the proof of Theorem 2 in~\cite{Neely2008DelayMM}.
We reproduce it with some minor revisions for this paper to be self-contained.

Let $Y_t\!=\!Q(t)$, then Then $Y_t$ is a positive recurrent Markov chain (proved in~\autoref{subsec:throughput-analysis}). Define $V, f, g: \mathcal{Y}\rightarrow \mathbf{N}^{+}$ such that,
\begin{align*}
V(Y_t) &= L(Y_t)\\ f(Y_t)&=-2\sum_{ij}q_{ij}(t)\big{(}D^\dagger_{ij}(t)-A^\dagger_{ij}(t)\big{)}\\
g(Y_t)&=\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}.
\end{align*}
Then, $V, f, q$ defined above satisfy~\autoref{eq:mbreq} by using~\autoref{eq:uncond-drift}.

Using~\autoref{thm:moment-bound}, we have,
\begin{eqnarray}
\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[f(Y_t)]\!\leq\! \lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[g(Y_t)].\label{eq:bound-ineq}
\end{eqnarray}

With~\autoref{eq:bounded-first-term}, we have,
\begin{align}
\mathbf{E}[f(Y_t)]
&=\mathbf{E}\Big{[}-2\sum_{ij}q_{ij}(t)\big{(}D^\dagger_{ij}(t)-A^\dagger_{ij}(t)\big{)}\Big{]}\nonumber\\
&=\mathbf{E}\Big{[}\mathbf{E}\Big{[}-2\sum_{ij}q_{ij}(t)\big{(}D^\dagger_{ij}(t)-A^\dagger_{ij}(t)\big{)}\mid Q(t) \Big{]}\Big{]}\nonumber\\
&\geq\mathbf{E}\big{[}-2(2\rho-1)\|Q(t)\|_1\big{]}\nonumber\\
&=-2(2\rho-1)\mathbf{E}[\|Q(t)\|_1]\nonumber\\
&=2(1-2\rho)\mathbf{E}[\|Q(t)\|_1]. \label{eq:delay-part-1}
\end{align}
With~\autoref{eq:for-delay-analysis} in the remarks of proof of~\autoref{thm:stability-qps}, we have,
\begin{align}
\mathbf{E}[g(Y_t)]&=\mathbf{E}\Big{[}\sum_{ij}\big{(}a_{ij}(t)-d_{ij}(t)\big{)}\big{(}A^\dagger_{ij}(t)-D^\dagger_{ij}(t)\big{)}\Big{]}\nonumber\\
&\leq \sigma^2_{ij}\!-\!\lambda_{ij}\Lambda^\dagger_{ij}\!+\!\lambda_{ij}.\label{eq:delay-part-2}
\end{align}

Combine~\autoref{eq:delay-part-1}, ~\autoref{eq:delay-part-2} and~\autoref{eq:bound-ineq}, we have,
\begin{align}
\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}2(1-2\rho)\mathbf{E}[\|Q(t)\|_1]
&\leq\lim\limits_{T\rightarrow\infty}\frac{1}{T}\mathbf{E}[g(Y_t)]\nonumber\\
&\leq\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{n=0}^{T-1}\mathbf{E}[g(Y_t)]\nonumber\\
&\leq\sigma^2_{ij}\!-\!\lambda_{ij}\Lambda^\dagger_{ij}\!+\!\lambda_{ij}.\nonumber
\end{align}
\end{comment}

% Therefore, we have,
% \begin{equation*}\label{eq:final-delay-bound}
% \lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[\|Q(t)\|_1]\leq\frac{1}{2(1-2\rho)}\sum_{i,j}\big{(}\sigma^2_{ij}\!-\!\lambda_{ij}\Lambda^\dagger_{ij}\!+\!\lambda_{ij}\big{)}.
% \end{equation*}

Therefore, we have, in steady state, 
\begin{equation*}%\label{eq:final-delay-bound}
\mathbf{E}[\|\bar{Q}\|_1]\leq\frac{1}{2(1-2\rho)}\sum_{i,j}\big{(}\sigma^2_{ij}\!-\!\lambda_{ij}\Lambda^\dagger_{ij}\!+\!\lambda_{ij}\big{)}.
\end{equation*}
\end{proof}
It is not hard to check (by applying Little's Law) that the average delay (experienced by packets) is
bounded by a constant independent of $N$ ({\it i.e., order-optimal}) for a given maximum load factor $\rho<1/2$,
if the variance $\sigma^2_{ij}$ for any $i,j$ is assumed to be finite.
For the special case of Bernoulli {\it i.i.d.} arrival (when $\sigma^2_{ij}=\lambda_{ij}-\lambda^2_{ij}$),
this bound (the RHS) can be further tightened to $\frac{\sum_{i,j}\lambda_{ij}}{1-2\rho}$.  This implies, by Little's Law, the following ``clean'' bound: $\bar{\omega}\leq \frac{1}{1-2\rho}$
where $\bar{\omega}$ is 
% the total of the long-run average delays of all $N^2$ VOQs 
the expected delay averaged over
all packets transmitting through the switch.
% Finally, using exactly the same $f$ and $g$, we have derived for QPS-1 the same delay
% bounds as derived in~\mbox{\cite{Neely2008DelayMM,Neely2009MMDelay}} for maximal matchings under
% other traffic arrival processes ({\it e.g.}, the bursty ON/OFF process).


%Note that by using similar approaches as in~\cite{Neely2008DelayMM,Neely2009MMDelay},
%we can further obtain the exact same delay bounds, which were derived for the maximal matchings
%in~\cite{Neely2008DelayMM,Neely2009MMDelay}, for QPS-r.



% From~\autoref{eq:bt}, $\bar{d}_{ij}\triangleq\lim_{T\rightarrow\infty}\frac{1}{T}\sum_{t=0}^{T-1}\mathbf{E}[d_{ij}(t)]=\lambda_{ij}$ (as $\{Q(t),S(t)\}_{t=0}^{\infty}$ is positive recurrent), we have,
% \begin{equation}
% 2(1-2\rho)\sum_{ij}\hat{q}_{ij}\leq f(\hat{Y}) \leq g(\hat{Y}) \leq \sum_{ij}\big{(}\sigma^2_{ij}-\lambda_{ij}\Lambda^\dagger_{ij} + \lambda_{ij}\big{)}.
% \end{equation}

% Note that $\sum_{ij}\bar{q}_{ij}=\sum_{ij}\hat{q}_{ij}$, therefore,
% \begin{equation}
% \sum_{ij}\bar{q}_{ij}\leq \frac{\sum_{ij}\big{(}\sigma^2_{ij}-\lambda_{ij}\Lambda^\dagger_{ij} + \lambda_{ij}\big{)}}{2(1-2\rho)}.
% \end{equation}



% \end{IEEEproof}
\begin{comment}
\noindent
{\bf Discussion.}  For the special case of Bernoulli {\it i.i.d.} traffic arrivals (when $\sigma^2_{ij}=\lambda_{ij}-\lambda^2_{ij}$),
the RHS of~autoref{eq:final-delay-bound} can be further simplified as $\frac{\sum_{i,j}\lambda_{ij}}{1-2\rho}$.  This implies, by Little's Law, that
$\bar{\omega}\leq \frac{1}{1-2\rho}$, where $\bar{\omega}$ is the sum of the long term average delays of all $N^2$ VOQs.




Note that For Bernoulli {\it i.i.d.} traffic, we have $\sigma^2_{ij}=\lambda_{ij}-\lambda^2_{ij}$, hence,
\begin{align}
&\lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum_{n=0}^{T-1}\mathbf{E}[\|Q(t)\|_1]\nonumber\\
\leq&\frac{1}{2(1-2\rho)}\sum_{i,j}\big{(}\sigma^2_{ij}-\lambda_{ij}\Lambda^\dagger_{ij} + \lambda_{ij}\big{)}\nonumber\\
=&\frac{1}{2(1-2\rho)}\sum_{i,j}\big{(}\sigma^2_{ij}-\lambda_{ij}(\Lambda_{i*}+\Lambda_{*j} -\lambda_{ij})+ \lambda_{ij}\big{)}.\nonumber\\
\leq&\frac{1}{2 (1 \!-\! 2\rho)}\sum_{i,j}\big{(}\sigma^2_{ij} \!+\! \lambda^2_{ij} \!+\! \lambda_{ij}\big{)} \nonumber\\
=&\frac{\sum_{i,j}\lambda_{ij}}{1-2\rho}.
\end{align}

By Little's Law, we can derive the average waiting delay under Bernoulli {\it i.i.d.} traffic satisfies
\begin{equation}\label{eq:delay-bound}\bar{\omega}\leq \frac{1}{1-2\rho}.\end{equation}
Clearly it is independent of switch size, $N$.

\end{comment}

